Universal Approximation in Dropout Neural Networks

We prove two universal approximation theorems for a range of dropout neural networks. These are feed-forward neural networks in which each edge is given a random $\{0,1\}$-valued filter, that have two modes of operation: in the first each edge output is multiplied by its random filter, resulting in a random output, while in the second each edge output is multiplied by the expectation of its filter, leading to a deterministic output. It is common to use the random mode during training and the deterministic mode during testing and prediction. Both theorems are of the following form: Given a function to approximate and a threshold $\varepsilon>0$, there exists a dropout network that is $\varepsilon$-close in probability and in $L^q$. The first theorem applies to dropout networks in the random mode. It assumes little on the activation function, applies to a wide class of networks, and can even be applied to approximation schemes other than neural networks. The core is an algebraic property that shows that deterministic networks can be exactly matched in expectation by random networks. The second theorem makes stronger assumptions and gives a stronger result. Given a function to approximate, it provides existence of a network that approximates in both modes simultaneously. Proof components are a recursive replacement of edges by independent copies, and a special first-layer replacement that couples the resulting larger network to the input. The functions to be approximated are assumed to be elements of general normed spaces, and the approximations are measured in the corresponding norms. The networks are constructed explicitly. Because of the different methods of proof, the two results give independent insight into the approximation properties of random dropout networks. With this, we establish that dropout neural networks broadly satisfy a universal-approximation property.

==> images/raw_data_of_M_curves.tex <==
% Start of data.

% Final RV 1.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0732086) (-9.9,0.0731932) (-9.8,0.0731752) (-9.7,0.0731543) (-9.6,0.0731308) (-9.5,0.0731027) (-9.4,0.0730708) (-9.3,0.0730334) (-9.2,0.0729905) (-9.1,0.0729405) (-9.,0.0728828) (-8.9,0.072816) (-8.8,0.0727389) (-8.7,0.0726497) (-8.6,0.0725458) (-8.5,0.0724256) (-8.4,0.0722872) (-8.3,0.0721262) (-8.2,0.0719405) (-8.1,0.0717258) (-8.,0.0714774) (-7.9,0.0711896) (-7.8,0.0708569) (-7.7,0.0704719) (-7.6,0.0700269) (-7.5,0.0695125) (-7.4,0.0689174) (-7.3,0.0682295) (-7.2,0.0674348) (-7.1,0.0665168) (-7.,0.0654563) (-6.9,0.0642324) (-6.8,0.062819) (-6.7,0.0611893) (-6.6,0.0593097) (-6.5,0.0571445) (-6.4,0.0546499) (-6.3,0.0517802) (-6.2,0.0484807) (-6.1,0.0446907) (-6.,0.0403425) (-5.9,0.0353607) (-5.8,0.0296614) (-5.7,0.0231526) (-5.6,0.0157353) (-5.5,0.00730306) (-5.4,-0.00225709) (-5.3,-0.0130601) (-5.2,-0.0252199) (-5.1,-0.0388461) (-5.,-0.0540308) (-4.9,-0.0708438) (-4.8,-0.0893141) (-4.7,-0.109413) (-4.6,-0.131027) (-4.5,-0.153933) (-4.4,-0.177756) (-4.3,-0.201935) (-4.2,-0.225676) (-4.1,-0.247914) (-4.,-0.267286) (-3.9,-0.28213) (-3.8,-0.290525) (-3.7,-0.290405) (-3.6,-0.279757) (-3.5,-0.256911) (-3.4,-0.220906) (-3.3,-0.171878) (-3.2,-0.111334) (-3.1,-0.0422253) (-3.,0.0312946) (-2.9,0.104422) (-2.8,0.172427) (-2.7,0.231363) (-2.6,0.278557) (-2.5,0.312775) (-2.4,0.334112) (-2.3,0.343675) (-2.2,0.343196) (-2.1,0.334685) (-2.,0.320154) (-1.9,0.30145) (-1.8,0.280148) (-1.7,0.25753) (-1.6,0.234585) (-1.5,0.212047) (-1.4,0.190432) (-1.3,0.170075) (-1.2,0.151177) (-1.1,0.133833) (-1.,0.118063) (-0.9,0.103835) (-0.8,0.0910774) (-0.7,0.0796998) (-0.6,0.0695977) (-0.5,0.0606624) (-0.4,0.052784) (-0.3,0.0458567) (-0.2,0.03978) (-0.1,0.03446) (0.,0.0298108) (0.1,0.0257536) (0.2,0.0222179) (0.3,0.0191399) (0.4,0.0164631) (0.5,0.0141372) (0.6,0.0121176) (0.7,0.0103651) (0.8,0.00884539) (0.9,0.00752804) (1.,0.00638663) (1.1,0.00539807) (1.2,0.00454214) (1.3,0.00380129) (1.4,0.00316018) (1.5,0.00260553) (1.6,0.00212577) (1.7,0.00171085) (1.8,0.00135207) (1.9,0.00104187) (2.,0.00077371) (2.1,0.000541912) (2.2,0.000341562) (2.3,0.000168412) (2.4,0.0000187769) (2.5,-0.000110528) (2.6,-0.000222258) (2.7,-0.0003188) (2.8,-0.000402212) (2.9,-0.000474278) (3.,-0.000536539) (3.1,-0.000590328) (3.2,-0.000636796) (3.3,-0.000676938) (3.4,-0.000711616) (3.5,-0.000741572) (3.6,-0.000767452) (3.7,-0.000789803) (3.8,-0.000809114) (3.9,-0.000825795) (4.,-0.000840198) (4.1,-0.000852645) (4.2,-0.000863395) (4.3,-0.000872681) (4.4,-0.000880699) (4.5,-0.000887628) (4.6,-0.000893614) (4.7,-0.000898783) (4.8,-0.000903247) (4.9,-0.000907101) (5.,-0.00091043) (5.1,-0.000913311) (5.2,-0.000915794) (5.3,-0.00091794) (5.4,-0.000919797) (5.5,-0.000921393) (5.6,-0.000922777) (5.7,-0.000923975) (5.8,-0.000925007) (5.9,-0.000925896) (6.,-0.000926666) (6.1,-0.000927331) (6.2,-0.000927906) (6.3,-0.000928402) (6.4,-0.000928831) (6.5,-0.000929199) (6.6,-0.000929521) (6.7,-0.000929797) (6.8,-0.000930033) (6.9,-0.000930241) (7.,-0.000930416) (7.1,-0.000930569) (7.2,-0.000930702) (7.3,-0.000930818) (7.4,-0.00093092) (7.5,-0.000931001) (7.6,-0.000931077) (7.7,-0.000931142) (7.8,-0.000931196) (7.9,-0.000931246) (8.,-0.000931286) (8.1,-0.000931323) (8.2,-0.000931352) (8.3,-0.000931378) (8.4,-0.000931403) (8.5,-0.000931419) (8.6,-0.000931439) (8.7,-0.000931454) (8.8,-0.000931467) (8.9,-0.000931479) (9.,-0.000931484) (9.1,-0.000931494) (9.2,-0.000931499) (9.3,-0.000931508) (9.4,-0.00093151) (9.5,-0.000931518) (9.6,-0.000931521) (9.7,-0.000931522) (9.8,-0.000931525) (9.9,-0.000931532) (10.,-0.000931534) 
};

% Final RV 2.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.000839666) (-9.9,0.000825316) (-9.8,0.00080853) (-9.7,0.00078905) (-9.6,0.000767125) (-9.5,0.000740953) (-9.4,0.000711208) (-9.3,0.00067639) (-9.2,0.000636391) (-9.1,0.000589788) (-9.,0.000536015) (-8.9,0.000473788) (-8.8,0.000401905) (-8.7,0.000318768) (-8.6,0.000221936) (-8.5,0.000109863) (-8.4,-0.000019094) (-8.3,-0.000169102) (-8.2,-0.000342185) (-8.1,-0.000542309) (-8.,-0.000773758) (-7.9,-0.00104195) (-7.8,-0.00135203) (-7.7,-0.00171083) (-7.6,-0.00212546) (-7.5,-0.00260476) (-7.4,-0.00315934) (-7.3,-0.00380035) (-7.2,-0.00454071) (-7.1,-0.00539609) (-7.,-0.00638407) (-6.9,-0.00752427) (-6.8,-0.00884088) (-6.7,-0.0103589) (-6.6,-0.0121095) (-6.5,-0.0141261) (-6.4,-0.0164491) (-6.3,-0.0191211) (-6.2,-0.0221928) (-6.1,-0.0257207) (-6.,-0.0297675) (-5.9,-0.034403) (-5.8,-0.039705) (-5.7,-0.0457582) (-5.6,-0.0526542) (-5.5,-0.0604911) (-5.4,-0.0693725) (-5.3,-0.0794036) (-5.2,-0.0906877) (-5.1,-0.103324) (-5.,-0.117393) (-4.9,-0.132955) (-4.8,-0.15003) (-4.7,-0.168581) (-4.6,-0.18849) (-4.5,-0.209535) (-4.4,-0.231346) (-4.3,-0.253376) (-4.2,-0.274857) (-4.1,-0.29476) (-4.,-0.311773) (-3.9,-0.324299) (-3.8,-0.330495) (-3.7,-0.328385) (-3.6,-0.316044) (-3.5,-0.291881) (-3.4,-0.254991) (-3.3,-0.20552) (-3.2,-0.144938) (-3.1,-0.0760974) (-3.,-0.00300679) (-2.9,0.0697005) (-2.8,0.137463) (-2.7,0.196473) (-2.6,0.244141) (-2.5,0.279266) (-2.4,0.301923) (-2.3,0.313158) (-2.2,0.314626) (-2.1,0.308248) (-2.,0.295952) (-1.9,0.27951) (-1.8,0.260438) (-1.7,0.239969) (-1.6,0.219063) (-1.5,0.198429) (-1.4,0.17857) (-1.3,0.15982) (-1.2,0.142379) (-1.1,0.126346) (-1.,0.11175) (-0.9,0.0985674) (-0.8,0.0867374) (-0.7,0.0761796) (-0.6,0.0667998) (-0.5,0.0584992) (-0.4,0.0511773) (-0.3,0.044737) (-0.2,0.0390856) (-0.1,0.0341368) (0.,0.0298108) (0.1,0.0260349) (0.2,0.0227438) (0.3,0.0198783) (0.4,0.017386) (0.5,0.01522) (0.6,0.0133391) (0.7,0.011707) (0.8,0.0102913) (0.9,0.00906419) (1.,0.00800086) (1.1,0.00707986) (1.2,0.00628241) (1.3,0.00559213) (1.4,0.00499476) (1.5,0.00447793) (1.6,0.00403088) (1.7,0.00364423) (1.8,0.00330989) (1.9,0.00302082) (2.,0.00277092) (2.1,0.00255489) (2.2,0.00236818) (2.3,0.00220681) (2.4,0.00206736) (2.5,0.00194685) (2.6,0.00184272) (2.7,0.00175274) (2.8,0.001675) (2.9,0.00160784) (3.,0.00154981) (3.1,0.00149968) (3.2,0.00145637) (3.3,0.00141895) (3.4,0.00138663) (3.5,0.00135871) (3.6,0.00133459) (3.7,0.00131376) (3.8,0.00129576) (3.9,0.00128021) (4.,0.00126679) (4.1,0.00125519) (4.2,0.00124517) (4.3,0.00123651) (4.4,0.00122904) (4.5,0.00122258) (4.6,0.001217) (4.7,0.00121219) (4.8,0.00120802) (4.9,0.00120443) (5.,0.00120133) (5.1,0.00119864) (5.2,0.00119633) (5.3,0.00119433) (5.4,0.0011926) (5.5,0.00119111) (5.6,0.00118982) (5.7,0.0011887) (5.8,0.00118774) (5.9,0.00118691) (6.,0.00118619) (6.1,0.00118558) (6.2,0.00118504) (6.3,0.00118458) (6.4,0.00118418) (6.5,0.00118383) (6.6,0.00118353) (6.7,0.00118328) (6.8,0.00118306) (6.9,0.00118286) (7.,0.0011827) (7.1,0.00118256) (7.2,0.00118243) (7.3,0.00118232) (7.4,0.00118223) (7.5,0.00118215) (7.6,0.00118208) (7.7,0.00118202) (7.8,0.00118197) (7.9,0.00118193) (8.,0.00118189) (8.1,0.00118186) (8.2,0.00118183) (8.3,0.0011818) (8.4,0.00118178) (8.5,0.00118176) (8.6,0.00118175) (8.7,0.00118173) (8.8,0.00118172) (8.9,0.00118171) (9.,0.0011817) (9.1,0.0011817) (9.2,0.00118169) (9.3,0.00118168) (9.4,0.00118168) (9.5,0.00118167) (9.6,0.00118167) (9.7,0.00118167) (9.8,0.00118166) (9.9,0.00118166) (10.,0.00118166) 
};

% Final RV 3.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.164388) (-9.9,0.164372) (-9.8,0.164355) (-9.7,0.164335) (-9.6,0.164312) (-9.5,0.164284) (-9.4,0.164253) (-9.3,0.164218) (-9.2,0.164175) (-9.1,0.164127) (-9.,0.164071) (-8.9,0.164006) (-8.8,0.16393) (-8.7,0.163844) (-8.6,0.163743) (-8.5,0.163626) (-8.4,0.163491) (-8.3,0.163334) (-8.2,0.163154) (-8.1,0.162945) (-8.,0.162703) (-7.9,0.162423) (-7.8,0.162099) (-7.7,0.161725) (-7.6,0.161291) (-7.5,0.16079) (-7.4,0.160211) (-7.3,0.159542) (-7.2,0.158768) (-7.1,0.157875) (-7.,0.156842) (-6.9,0.155651) (-6.8,0.154274) (-6.7,0.152688) (-6.6,0.150857) (-6.5,0.148748) (-6.4,0.146318) (-6.3,0.143523) (-6.2,0.140308) (-6.1,0.136614) (-6.,0.132375) (-5.9,0.127517) (-5.8,0.121958) (-5.7,0.115608) (-5.6,0.108368) (-5.5,0.100134) (-5.4,0.0907931) (-5.3,0.0802312) (-5.2,0.0683343) (-5.1,0.0549909) (-5.,0.0401052) (-4.9,0.0236022) (-4.8,0.00544366) (-4.7,-0.0143551) (-4.6,-0.0356994) (-4.5,-0.058392) (-4.4,-0.0820946) (-4.3,-0.106292) (-4.2,-0.130253) (-4.1,-0.152986) (-4.,-0.173222) (-3.9,-0.189408) (-3.8,-0.199741) (-3.7,-0.202284) (-3.6,-0.195139) (-3.5,-0.176726) (-3.4,-0.146127) (-3.3,-0.103443) (-3.2,-0.0500581) (-3.1,0.011293) (-3.,0.0767523) (-2.9,0.141852) (-2.8,0.202195) (-2.7,0.254115) (-2.6,0.295137) (-2.5,0.32413) (-2.4,0.341208) (-2.3,0.347422) (-2.2,0.34441) (-2.1,0.334061) (-2.,0.318263) (-1.9,0.298745) (-1.8,0.276978) (-1.7,0.254155) (-1.6,0.231194) (-1.5,0.208769) (-1.4,0.187354) (-1.3,0.16725) (-1.2,0.148633) (-1.1,0.131581) (-1.,0.116101) (-0.9,0.102151) (-0.8,0.0896578) (-0.7,0.0785255) (-0.6,0.0686486) (-0.5,0.059918) (-0.4,0.0522243) (-0.3,0.0454624) (-0.2,0.0395332) (-0.1,0.0343442) (0.,0.0298108) (0.1,0.0258557) (0.2,0.0224097) (0.3,0.0194104) (0.4,0.0168025) (0.5,0.0145368) (0.6,0.0125698) (0.7,0.0108632) (0.8,0.00938326) (0.9,0.0081006) (1.,0.00698933) (1.1,0.00602694) (1.2,0.00519373) (1.3,0.00447258) (1.4,0.00384855) (1.5,0.00330869) (1.6,0.00284175) (1.7,0.00243794) (1.8,0.00208876) (1.9,0.00178688) (2.,0.00152592) (2.1,0.00130034) (2.2,0.00110538) (2.3,0.000936881) (2.4,0.000791272) (2.5,0.000665448) (2.6,0.000556727) (2.7,0.000462786) (2.8,0.000381621) (2.9,0.000311498) (3.,0.000250916) (3.1,0.000198577) (3.2,0.000153363) (3.3,0.000114303) (3.4,0.0000805619) (3.5,0.0000514139) (3.6,0.000026233) (3.7,0.00000448381) (3.8,-0.0000143048) (3.9,-0.0000305341) (4.,-0.0000445505) (4.1,-0.0000566605) (4.2,-0.0000671202) (4.3,-0.0000761549) (4.4,-0.0000839575) (4.5,-0.000090698) (4.6,-0.0000965216) (4.7,-0.000101551) (4.8,-0.000105895) (4.9,-0.000109645) (5.,-0.000112886) (5.1,-0.000115687) (5.2,-0.000118103) (5.3,-0.000120191) (5.4,-0.000121997) (5.5,-0.000123553) (5.6,-0.000124899) (5.7,-0.000126063) (5.8,-0.000127067) (5.9,-0.000127933) (6.,-0.000128682) (6.1,-0.000129329) (6.2,-0.000129888) (6.3,-0.000130371) (6.4,-0.000130788) (6.5,-0.000131146) (6.6,-0.000131459) (6.7,-0.000131727) (6.8,-0.000131958) (6.9,-0.00013216) (7.,-0.000132331) (7.1,-0.000132481) (7.2,-0.00013261) (7.3,-0.000132722) (7.4,-0.00013282) (7.5,-0.000132901) (7.6,-0.000132974) (7.7,-0.000133037) (7.8,-0.000133089) (7.9,-0.000133137) (8.,-0.000133177) (8.1,-0.000133212) (8.2,-0.000133241) (8.3,-0.000133266) (8.4,-0.000133289) (8.5,-0.000133307) (8.6,-0.000133325) (8.7,-0.000133339) (8.8,-0.000133352) (8.9,-0.000133363) (9.,-0.000133371) (9.1,-0.00013338) (9.2,-0.000133385) (9.3,-0.000133393) (9.4,-0.000133396) (9.5,-0.000133403) (9.6,-0.000133406) (9.7,-0.000133408) (9.8,-0.00013341) (9.9,-0.000133415) (10.,-0.000133417) 
};

% Final RV 4.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,-0.0105675) (-9.9,-0.010582) (-9.8,-0.0105989) (-9.7,-0.0106186) (-9.6,-0.0106407) (-9.5,-0.0106671) (-9.4,-0.0106971) (-9.3,-0.0107322) (-9.2,-0.0107725) (-9.1,-0.0108195) (-9.,-0.0108738) (-8.9,-0.0109365) (-8.8,-0.0110091) (-8.7,-0.011093) (-8.6,-0.0111906) (-8.5,-0.0113037) (-8.4,-0.0114337) (-8.3,-0.0115851) (-8.2,-0.0117596) (-8.1,-0.0119615) (-8.,-0.012195) (-7.9,-0.0124655) (-7.8,-0.0127783) (-7.7,-0.0131402) (-7.6,-0.0135585) (-7.5,-0.0140419) (-7.4,-0.0146013) (-7.3,-0.0152478) (-7.2,-0.0159947) (-7.1,-0.0168574) (-7.,-0.017854) (-6.9,-0.019004) (-6.8,-0.0203321) (-6.7,-0.021863) (-6.6,-0.0236288) (-6.5,-0.0256627) (-6.4,-0.0280056) (-6.3,-0.0307006) (-6.2,-0.0337985) (-6.1,-0.0373565) (-6.,-0.0414375) (-5.9,-0.0461123) (-5.8,-0.0514588) (-5.7,-0.0575627) (-5.6,-0.0645161) (-5.5,-0.0724178) (-5.4,-0.0813721) (-5.3,-0.0914845) (-5.2,-0.102859) (-5.1,-0.115595) (-5.,-0.129774) (-4.9,-0.145454) (-4.8,-0.162655) (-4.7,-0.181339) (-4.6,-0.201384) (-4.5,-0.222563) (-4.4,-0.244501) (-4.3,-0.266642) (-4.2,-0.288207) (-4.1,-0.308151) (-4.,-0.325145) (-3.9,-0.33757) (-3.8,-0.343558) (-3.7,-0.341109) (-3.6,-0.328271) (-3.5,-0.303437) (-3.4,-0.265689) (-3.3,-0.215181) (-3.2,-0.153403) (-3.1,-0.0832504) (-3.,-0.00878845) (-2.9,0.0652841) (-2.8,0.134342) (-2.7,0.194521) (-2.6,0.243197) (-2.5,0.279147) (-2.4,0.302447) (-2.3,0.314153) (-2.2,0.315942) (-2.1,0.309757) (-2.,0.297555) (-1.9,0.281128) (-1.8,0.262016) (-1.7,0.241468) (-1.6,0.220455) (-1.5,0.199701) (-1.4,0.179716) (-1.3,0.160838) (-1.2,0.143272) (-1.1,0.127121) (-1.,0.112414) (-0.9,0.099129) (-0.8,0.0872056) (-0.7,0.0765632) (-0.6,0.0671073) (-0.5,0.0587388) (-0.4,0.0513564) (-0.3,0.0448625) (-0.2,0.0391638) (-0.1,0.0341733) (0.,0.0298108) (0.1,0.0260029) (0.2,0.0226837) (0.3,0.0197938) (0.4,0.0172801) (0.5,0.0150956) (0.6,0.0131986) (0.7,0.0115523) (0.8,0.0101245) (0.9,0.00888674) (1.,0.00781422) (1.1,0.00688525) (1.2,0.00608089) (1.3,0.00538462) (1.4,0.00478207) (1.5,0.00426076) (1.6,0.00380982) (1.7,0.00341982) (1.8,0.00308257) (1.9,0.00279098) (2.,0.00253891) (2.1,0.002321) (2.2,0.00213267) (2.3,0.00196989) (2.4,0.00182922) (2.5,0.00170766) (2.6,0.00160262) (2.7,0.00151186) (2.8,0.00143344) (2.9,0.00136569) (3.,0.00130716) (3.1,0.00125659) (3.2,0.0012129) (3.3,0.00117516) (3.4,0.00114256) (3.5,0.0011144) (3.6,0.00109006) (3.7,0.00106905) (3.8,0.0010509) (3.9,0.00103521) (4.,0.00102167) (4.1,0.00100997) (4.2,0.000999862) (4.3,0.000991131) (4.4,0.000983592) (4.5,0.000977079) (4.6,0.000971452) (4.7,0.000966593) (4.8,0.000962395) (4.9,0.00095877) (5.,0.000955639) (5.1,0.000952933) (5.2,0.000950597) (5.3,0.000948579) (5.4,0.000946835) (5.5,0.000945332) (5.6,0.000944031) (5.7,0.000942907) (5.8,0.000941936) (5.9,0.000941099) (6.,0.000940376) (6.1,0.00093975) (6.2,0.00093921) (6.3,0.000938743) (6.4,0.000938341) (6.5,0.000937994) (6.6,0.000937692) (6.7,0.000937432) (6.8,0.000937209) (6.9,0.000937015) (7.,0.000936848) (7.1,0.000936704) (7.2,0.000936579) (7.3,0.000936471) (7.4,0.000936377) (7.5,0.000936297) (7.6,0.000936228) (7.7,0.000936167) (7.8,0.000936117) (7.9,0.00093607) (8.,0.000936032) (8.1,0.000935999) (8.2,0.00093597) (8.3,0.000935946) (8.4,0.000935923) (8.5,0.000935905) (8.6,0.000935889) (8.7,0.000935876) (8.8,0.000935863) (8.9,0.000935853) (9.,0.000935844) (9.1,0.000935836) (9.2,0.00093583) (9.3,0.000935823) (9.4,0.00093582) (9.5,0.000935815) (9.6,0.000935811) (9.7,0.000935809) (9.8,0.000935805) (9.9,0.000935803) (10.,0.0009358) 
};

% Final RV 5.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.186477) (-9.9,0.186461) (-9.8,0.186443) (-9.7,0.186421) (-9.6,0.186397) (-9.5,0.186368) (-9.4,0.186336) (-9.3,0.186298) (-9.2,0.186253) (-9.1,0.186202) (-9.,0.186143) (-8.9,0.186075) (-8.8,0.185995) (-8.7,0.185903) (-8.6,0.185797) (-8.5,0.185674) (-8.4,0.185532) (-8.3,0.185366) (-8.2,0.185176) (-8.1,0.184955) (-8.,0.1847) (-7.9,0.184405) (-7.8,0.184063) (-7.7,0.183668) (-7.6,0.183211) (-7.5,0.182683) (-7.4,0.182072) (-7.3,0.181366) (-7.2,0.18055) (-7.1,0.179608) (-7.,0.178518) (-6.9,0.177262) (-6.8,0.17581) (-6.7,0.174136) (-6.6,0.172205) (-6.5,0.169981) (-6.4,0.167417) (-6.3,0.164468) (-6.2,0.161076) (-6.1,0.157179) (-6.,0.152707) (-5.9,0.147582) (-5.8,0.141716) (-5.7,0.135016) (-5.6,0.127376) (-5.5,0.118686) (-5.4,0.108828) (-5.3,0.09768) (-5.2,0.0851214) (-5.1,0.0710341) (-5.,0.055316) (-4.9,0.0378868) (-4.8,0.0187044) (-4.7,-0.00221663) (-4.6,-0.0247792) (-4.5,-0.0487786) (-4.4,-0.0738619) (-4.3,-0.099491) (-4.2,-0.1249) (-4.1,-0.149053) (-4.,-0.170618) (-3.9,-0.187967) (-3.8,-0.199211) (-3.7,-0.202317) (-3.6,-0.195294) (-3.5,-0.176481) (-3.4,-0.144914) (-3.3,-0.100694) (-3.2,-0.045268) (-3.1,0.0185018) (-3.,0.0865754) (-2.9,0.154274) (-2.8,0.21699) (-2.7,0.270888) (-2.6,0.313373) (-2.5,0.343269) (-2.4,0.360693) (-2.3,0.366755) (-2.2,0.363173) (-2.1,0.351927) (-2.,0.335) (-1.9,0.314203) (-1.8,0.291079) (-1.7,0.266877) (-1.6,0.242557) (-1.5,0.218826) (-1.4,0.196178) (-1.3,0.174926) (-1.2,0.155254) (-1.1,0.13724) (-1.,0.120891) (-0.9,0.106161) (-0.8,0.092971) (-0.7,0.0812195) (-0.6,0.0707943) (-0.5,0.0615801) (-0.4,0.0534607) (-0.3,0.0463253) (-0.2,0.040069) (-0.1,0.0345939) (0.,0.0298108) (0.1,0.025638) (0.2,0.0220025) (0.3,0.0188384) (0.4,0.0160872) (0.5,0.013697) (0.6,0.011622) (0.7,0.00982174) (0.8,0.00826068) (0.9,0.00690766) (1.,0.00573546) (1.1,0.00472031) (1.2,0.00384143) (1.3,0.00308076) (1.4,0.00242253) (1.5,0.0018531) (1.6,0.00136058) (1.7,0.000934644) (1.8,0.000566349) (1.9,0.000247935) (2.,-0.0000273232) (2.1,-0.000265249) (2.2,-0.00047089) (2.3,-0.00064861) (2.4,-0.000802192) (2.5,-0.000934905) (2.6,-0.00104958) (2.7,-0.00114866) (2.8,-0.00123427) (2.9,-0.00130823) (3.,-0.00137213) (3.1,-0.00142733) (3.2,-0.00147502) (3.3,-0.00151622) (3.4,-0.00155181) (3.5,-0.00158255) (3.6,-0.00160911) (3.7,-0.00163205) (3.8,-0.00165187) (3.9,-0.00166899) (4.,-0.00168377) (4.1,-0.00169654) (4.2,-0.00170758) (4.3,-0.0017171) (4.4,-0.00172534) (4.5,-0.00173244) (4.6,-0.00173858) (4.7,-0.00174389) (4.8,-0.00174847) (4.9,-0.00175243) (5.,-0.00175585) (5.1,-0.0017588) (5.2,-0.00176135) (5.3,-0.00176355) (5.4,-0.00176545) (5.5,-0.0017671) (5.6,-0.00176852) (5.7,-0.00176974) (5.8,-0.0017708) (5.9,-0.00177172) (6.,-0.00177251) (6.1,-0.00177319) (6.2,-0.00177378) (6.3,-0.00177429) (6.4,-0.00177473) (6.5,-0.00177511) (6.6,-0.00177544) (6.7,-0.00177572) (6.8,-0.00177596) (6.9,-0.00177617) (7.,-0.00177635) (7.1,-0.00177651) (7.2,-0.00177665) (7.3,-0.00177677) (7.4,-0.00177687) (7.5,-0.00177696) (7.6,-0.00177703) (7.7,-0.0017771) (7.8,-0.00177715) (7.9,-0.0017772) (8.,-0.00177725) (8.1,-0.00177728) (8.2,-0.00177731) (8.3,-0.00177734) (8.4,-0.00177737) (8.5,-0.00177739) (8.6,-0.0017774) (8.7,-0.00177742) (8.8,-0.00177743) (8.9,-0.00177744) (9.,-0.00177745) (9.1,-0.00177746) (9.2,-0.00177747) (9.3,-0.00177747) (9.4,-0.00177748) (9.5,-0.00177748) (9.6,-0.00177749) (9.7,-0.00177749) (9.8,-0.00177749) (9.9,-0.0017775) (10.,-0.0017775) 
};

% Final RV 6.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0372542) (-9.9,0.0372392) (-9.8,0.0372217) (-9.7,0.0372014) (-9.6,0.0371786) (-9.5,0.0371513) (-9.4,0.0371203) (-9.3,0.0370839) (-9.2,0.0370422) (-9.1,0.0369937) (-9.,0.0369376) (-8.9,0.0368727) (-8.8,0.0367977) (-8.7,0.036711) (-8.6,0.03661) (-8.5,0.0364932) (-8.4,0.0363587) (-8.3,0.0362022) (-8.2,0.0360218) (-8.1,0.0358131) (-8.,0.0355717) (-7.9,0.035292) (-7.8,0.0349686) (-7.7,0.0345944) (-7.6,0.034162) (-7.5,0.0336621) (-7.4,0.0330838) (-7.3,0.0324152) (-7.2,0.0316431) (-7.1,0.0307509) (-7.,0.0297204) (-6.9,0.0285312) (-6.8,0.0271578) (-6.7,0.0255744) (-6.6,0.0237482) (-6.5,0.0216444) (-6.4,0.019221) (-6.3,0.0164331) (-6.2,0.013228) (-6.1,0.00954672) (-6.,0.00532359) (-5.9,0.000485519) (-5.8,-0.00504869) (-5.7,-0.0113681) (-5.6,-0.0185686) (-5.5,-0.026753) (-5.4,-0.0360301) (-5.3,-0.0465109) (-5.2,-0.0583046) (-5.1,-0.071516) (-5.,-0.0862328) (-4.9,-0.10252) (-4.8,-0.120401) (-4.7,-0.139845) (-4.6,-0.160734) (-4.5,-0.182844) (-4.4,-0.205801) (-4.3,-0.229048) (-4.2,-0.2518) (-4.1,-0.273001) (-4.,-0.291307) (-3.9,-0.30508) (-3.8,-0.312424) (-3.7,-0.311308) (-3.6,-0.299749) (-3.5,-0.276109) (-3.4,-0.239447) (-3.3,-0.189907) (-3.2,-0.128985) (-3.1,-0.0596011) (-3.,0.0141398) (-2.9,0.0874903) (-2.8,0.155777) (-2.7,0.2151) (-2.6,0.262811) (-2.5,0.297685) (-2.4,0.319809) (-2.3,0.330266) (-2.2,0.330758) (-2.1,0.323264) (-2.,0.309765) (-1.9,0.292082) (-1.8,0.271769) (-1.7,0.250093) (-1.6,0.228032) (-1.5,0.206313) (-1.4,0.185449) (-1.3,0.165775) (-1.2,0.147494) (-1.1,0.130704) (-1.,0.115428) (-0.9,0.101638) (-0.8,0.089269) (-0.7,0.0782341) (-0.6,0.0684335) (-0.5,0.0597629) (-0.4,0.0521162) (-0.3,0.0453915) (-0.2,0.0394916) (-0.1,0.0343258) (0.,0.0298108) (0.1,0.0258703) (0.2,0.022436) (0.3,0.0194461) (0.4,0.0168458) (0.5,0.0145861) (0.6,0.0126239) (0.7,0.0109213) (0.8,0.00944462) (0.9,0.00816461) (1.,0.0070555) (1.1,0.00609488) (1.2,0.00526314) (1.3,0.0045432) (1.4,0.00392018) (1.5,0.00338116) (1.6,0.00291493) (1.7,0.00251169) (1.8,0.00216302) (1.9,0.00186155) (2.,0.00160094) (2.1,0.00137566) (2.2,0.00118095) (2.3,0.00101266) (2.4,0.000867232) (2.5,0.000741562) (2.6,0.000632973) (2.7,0.000539145) (2.8,0.000458074) (2.9,0.000388032) (3.,0.000327521) (3.1,0.000275242) (3.2,0.00023008) (3.3,0.000191065) (3.4,0.000157361) (3.5,0.000128246) (3.6,0.000103093) (3.7,0.0000813684) (3.8,0.0000626005) (3.9,0.0000463894) (4.,0.0000323883) (4.1,0.0000202918) (4.2,0.00000984383) (4.3,0.000000818553) (4.4,-0.00000697583) (4.5,-0.0000137083) (4.6,-0.0000195254) (4.7,-0.0000245491) (4.8,-0.0000288884) (4.9,-0.0000326353) (5.,-0.0000358717) (5.1,-0.00003867) (5.2,-0.0000410842) (5.3,-0.0000431698) (5.4,-0.0000449734) (5.5,-0.0000465273) (5.6,-0.0000478721) (5.7,-0.0000490342) (5.8,-0.0000500376) (5.9,-0.0000509027) (6.,-0.000051651) (6.1,-0.0000522977) (6.2,-0.0000528558) (6.3,-0.0000533383) (6.4,-0.0000537552) (6.5,-0.0000541128) (6.6,-0.0000544248) (6.7,-0.000054694) (6.8,-0.0000549241) (6.9,-0.0000551257) (7.,-0.0000552968) (7.1,-0.0000554461) (7.2,-0.0000555758) (7.3,-0.000055687) (7.4,-0.0000557847) (7.5,-0.0000558667) (7.6,-0.0000559387) (7.7,-0.0000560013) (7.8,-0.0000560532) (7.9,-0.000056102) (8.,-0.0000561412) (8.1,-0.0000561758) (8.2,-0.0000562051) (8.3,-0.0000562303) (8.4,-0.000056254) (8.5,-0.0000562721) (8.6,-0.0000562891) (8.7,-0.000056303) (8.8,-0.0000563159) (8.9,-0.0000563267) (9.,-0.0000563344) (9.1,-0.0000563439) (9.2,-0.0000563498) (9.3,-0.0000563569) (9.4,-0.0000563608) (9.5,-0.000056366) (9.6,-0.0000563699) (9.7,-0.0000563718) (9.8,-0.0000563751) (9.9,-0.0000563782) (10.,-0.0000563816) 
};

% Final RV 7.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0508443) (-9.9,0.0508295) (-9.8,0.0508122) (-9.7,0.0507922) (-9.6,0.0507696) (-9.5,0.0507426) (-9.4,0.050712) (-9.3,0.0506761) (-9.2,0.0506349) (-9.1,0.0505869) (-9.,0.0505315) (-8.9,0.0504674) (-8.8,0.0503934) (-8.7,0.0503077) (-8.6,0.050208) (-8.5,0.0500925) (-8.4,0.0499597) (-8.3,0.0498051) (-8.2,0.0496269) (-8.1,0.0494207) (-8.,0.0491823) (-7.9,0.0489058) (-7.8,0.0485864) (-7.7,0.0482168) (-7.6,0.0477896) (-7.5,0.0472958) (-7.4,0.0467245) (-7.3,0.0460639) (-7.2,0.045301) (-7.1,0.0444198) (-7.,0.0434017) (-6.9,0.0422268) (-6.8,0.0408699) (-6.7,0.0393056) (-6.6,0.0375012) (-6.5,0.0354227) (-6.4,0.0330283) (-6.3,0.0302738) (-6.2,0.027107) (-6.1,0.0234695) (-6.,0.0192964) (-5.9,0.0145156) (-5.8,0.00904646) (-5.7,0.00280134) (-5.6,-0.00431497) (-5.5,-0.0124045) (-5.4,-0.0215749) (-5.3,-0.0319359) (-5.2,-0.043596) (-5.1,-0.0566594) (-5.,-0.0712141) (-4.9,-0.0873244) (-4.8,-0.105016) (-4.7,-0.12426) (-4.6,-0.144941) (-4.5,-0.166844) (-4.4,-0.1896) (-4.3,-0.212664) (-4.2,-0.235267) (-4.1,-0.256372) (-4.,-0.274662) (-3.9,-0.288525) (-3.8,-0.296101) (-3.7,-0.295393) (-3.6,-0.284451) (-3.5,-0.261663) (-3.4,-0.226103) (-3.3,-0.177908) (-3.2,-0.118545) (-3.1,-0.0508755) (-3.,0.02107) (-2.9,0.0926332) (-2.8,0.159228) (-2.7,0.217027) (-2.6,0.263432) (-2.5,0.297246) (-2.4,0.318556) (-2.3,0.328428) (-2.2,0.328537) (-2.1,0.320827) (-2.,0.307247) (-1.9,0.289583) (-1.8,0.269363) (-1.7,0.247829) (-1.6,0.225942) (-1.5,0.204413) (-1.4,0.183746) (-1.3,0.164267) (-1.2,0.146174) (-1.1,0.129561) (-1.,0.11445) (-0.9,0.100812) (-0.8,0.0885817) (-0.7,0.0776717) (-0.6,0.0679831) (-0.5,0.0594123) (-0.4,0.0518544) (-0.3,0.0452081) (-0.2,0.0393774) (-0.1,0.0342725) (0.,0.0298108) (0.1,0.025917) (0.2,0.0225236) (0.3,0.0195694) (0.4,0.0170001) (0.5,0.0147674) (0.6,0.0128289) (0.7,0.0111466) (0.8,0.00968775) (0.9,0.00842314) (1.,0.0073274) (1.1,0.00637837) (1.2,0.00555667) (1.3,0.00484543) (1.4,0.00422994) (1.5,0.00369744) (1.6,0.00323685) (1.7,0.0028385) (1.8,0.00249404) (1.9,0.00219622) (2.,0.00193877) (2.1,0.00171622) (2.2,0.00152387) (2.3,0.00135762) (2.4,0.00121396) (2.5,0.00108982) (2.6,0.000982546) (2.7,0.000889855) (2.8,0.000809767) (2.9,0.000740576) (3.,0.000680798) (3.1,0.000629155) (3.2,0.000584541) (3.3,0.000546) (3.4,0.000512703) (3.5,0.000483943) (3.6,0.000459095) (3.7,0.000437634) (3.8,0.000419095) (3.9,0.000403079) (4.,0.00038925) (4.1,0.000377299) (4.2,0.000366977) (4.3,0.000358063) (4.4,0.000350363) (4.5,0.000343712) (4.6,0.000337965) (4.7,0.000333002) (4.8,0.000328716) (4.9,0.000325015) (5.,0.000321817) (5.1,0.000319053) (5.2,0.000316669) (5.3,0.000314608) (5.4,0.000312826) (5.5,0.000311291) (5.6,0.000309962) (5.7,0.000308814) (5.8,0.000307823) (5.9,0.000306969) (6.,0.00030623) (6.1,0.000305591) (6.2,0.00030504) (6.3,0.000304563) (6.4,0.000304152) (6.5,0.000303797) (6.6,0.000303489) (6.7,0.000303225) (6.8,0.000302996) (6.9,0.000302798) (7.,0.000302629) (7.1,0.000302481) (7.2,0.000302354) (7.3,0.000302243) (7.4,0.000302147) (7.5,0.000302066) (7.6,0.000301995) (7.7,0.000301932) (7.8,0.000301881) (7.9,0.000301833) (8.,0.000301795) (8.1,0.000301759) (8.2,0.000301731) (8.3,0.000301706) (8.4,0.000301682) (8.5,0.000301665) (8.6,0.000301648) (8.7,0.000301634) (8.8,0.000301622) (8.9,0.00030161) (9.,0.000301604) (9.1,0.000301595) (9.2,0.000301588) (9.3,0.000301581) (9.4,0.000301578) (9.5,0.000301572) (9.6,0.000301569) (9.7,0.000301566) (9.8,0.000301564) (9.9,0.000301559) (10.,0.000301557) 
};

% Final RV 8.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,-0.14976) (-9.9,-0.149775) (-9.8,-0.149792) (-9.7,-0.149813) (-9.6,-0.149836) (-9.5,-0.149863) (-9.4,-0.149895) (-9.3,-0.149931) (-9.2,-0.149973) (-9.1,-0.150022) (-9.,-0.150078) (-8.9,-0.150144) (-8.8,-0.150219) (-8.7,-0.150307) (-8.6,-0.150408) (-8.5,-0.150526) (-8.4,-0.150661) (-8.3,-0.150819) (-8.2,-0.151001) (-8.1,-0.151211) (-8.,-0.151454) (-7.9,-0.151736) (-7.8,-0.152061) (-7.7,-0.152438) (-7.6,-0.152874) (-7.5,-0.153377) (-7.4,-0.153959) (-7.3,-0.154632) (-7.2,-0.155409) (-7.1,-0.156307) (-7.,-0.157343) (-6.9,-0.15854) (-6.8,-0.159921) (-6.7,-0.161514) (-6.6,-0.16335) (-6.5,-0.165464) (-6.4,-0.1679) (-6.3,-0.170701) (-6.2,-0.17392) (-6.1,-0.177615) (-6.,-0.181853) (-5.9,-0.186706) (-5.8,-0.192252) (-5.7,-0.198583) (-5.6,-0.205789) (-5.5,-0.213972) (-5.4,-0.223238) (-5.3,-0.233693) (-5.2,-0.245439) (-5.1,-0.258574) (-5.,-0.273172) (-4.9,-0.289285) (-4.8,-0.306917) (-4.7,-0.326011) (-4.6,-0.346416) (-4.5,-0.367865) (-4.4,-0.38993) (-4.3,-0.411984) (-4.2,-0.433158) (-4.1,-0.452294) (-4.,-0.467922) (-3.9,-0.478266) (-3.8,-0.481277) (-3.7,-0.474766) (-3.6,-0.456611) (-3.5,-0.425067) (-3.4,-0.379161) (-3.3,-0.319093) (-3.2,-0.246538) (-3.1,-0.164717) (-3.,-0.0781353) (-2.9,0.00800723) (-2.8,0.0885906) (-2.7,0.159332) (-2.6,0.21731) (-2.5,0.261148) (-2.4,0.290895) (-2.3,0.307686) (-2.2,0.31334) (-2.1,0.30998) (-2.,0.299744) (-1.9,0.284604) (-1.8,0.266252) (-1.7,0.246071) (-1.6,0.225139) (-1.5,0.204266) (-1.4,0.184027) (-1.3,0.164812) (-1.2,0.146863) (-1.1,0.130308) (-1.,0.115197) (-0.9,0.10152) (-0.8,0.0892245) (-0.7,0.0782352) (-0.6,0.0684599) (-0.5,0.0598005) (-0.4,0.0521553) (-0.3,0.0454255) (-0.2,0.0395164) (-0.1,0.0343388) (0.,0.0298108) (0.1,0.0258569) (0.2,0.0224093) (0.3,0.0194067) (0.4,0.0167942) (0.5,0.0145234) (0.6,0.0125511) (0.7,0.0108392) (0.8,0.00935415) (0.9,0.00806664) (1.,0.00695088) (1.1,0.00598435) (1.2,0.00514739) (1.3,0.00442285) (1.4,0.00379578) (1.5,0.00325321) (1.6,0.00278387) (1.7,0.00237792) (1.8,0.00202688) (1.9,0.00172335) (2.,0.00146093) (2.1,0.00123409) (2.2,0.00103802) (2.3,0.000868555) (2.4,0.000722101) (2.5,0.000595543) (2.6,0.000486182) (2.7,0.000391686) (2.8,0.000310038) (2.9,0.000239495) (3.,0.00017855) (3.1,0.000125896) (3.2,0.0000804086) (3.3,0.0000411124) (3.4,0.00000716587) (3.5,-0.0000221597) (3.6,-0.0000474937) (3.7,-0.0000693767) (3.8,-0.0000882796) (3.9,-0.000104608) (4.,-0.000118712) (4.1,-0.000130896) (4.2,-0.000141419) (4.3,-0.00015051) (4.4,-0.000158361) (4.5,-0.000165142) (4.6,-0.000171002) (4.7,-0.000176062) (4.8,-0.000180433) (4.9,-0.000184207) (5.,-0.000187467) (5.1,-0.000190285) (5.2,-0.000192718) (5.3,-0.000194819) (5.4,-0.000196634) (5.5,-0.0001982) (5.6,-0.000199555) (5.7,-0.000200725) (5.8,-0.000201736) (5.9,-0.000202607) (6.,-0.000203361) (6.1,-0.000204012) (6.2,-0.000204575) (6.3,-0.000205061) (6.4,-0.000205481) (6.5,-0.000205841) (6.6,-0.000206155) (6.7,-0.000206426) (6.8,-0.000206658) (6.9,-0.000206861) (7.,-0.000207034) (7.1,-0.000207184) (7.2,-0.000207315) (7.3,-0.000207426) (7.4,-0.000207525) (7.5,-0.000207608) (7.6,-0.00020768) (7.7,-0.000207743) (7.8,-0.000207796) (7.9,-0.000207844) (8.,-0.000207884) (8.1,-0.000207918) (8.2,-0.000207949) (8.3,-0.000207974) (8.4,-0.000207997) (8.5,-0.000208016) (8.6,-0.000208032) (8.7,-0.000208047) (8.8,-0.00020806) (8.9,-0.000208071) (9.,-0.000208079) (9.1,-0.000208088) (9.2,-0.000208094) (9.3,-0.000208101) (9.4,-0.000208105) (9.5,-0.00020811) (9.6,-0.000208114) (9.7,-0.000208116) (9.8,-0.00020812) (9.9,-0.000208122) (10.,-0.000208126) 
};

% Final RV 9.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0616722) (-9.9,0.0616565) (-9.8,0.0616383) (-9.7,0.0616171) (-9.6,0.0615932) (-9.5,0.0615647) (-9.4,0.0615324) (-9.3,0.0614945) (-9.2,0.0614509) (-9.1,0.0614002) (-9.,0.0613417) (-8.9,0.061274) (-8.8,0.0611956) (-8.7,0.0611052) (-8.6,0.0609998) (-8.5,0.0608779) (-8.4,0.0607375) (-8.3,0.0605742) (-8.2,0.0603859) (-8.1,0.0601679) (-8.,0.059916) (-7.9,0.0596241) (-7.8,0.0592866) (-7.7,0.0588961) (-7.6,0.0584446) (-7.5,0.0579228) (-7.4,0.0573191) (-7.3,0.0566214) (-7.2,0.0558153) (-7.1,0.0548841) (-7.,0.0538083) (-6.9,0.0525669) (-6.8,0.0511331) (-6.7,0.0494803) (-6.6,0.0475737) (-6.5,0.0453774) (-6.4,0.0428474) (-6.3,0.0399366) (-6.2,0.0365902) (-6.1,0.0327463) (-6.,0.0283365) (-5.9,0.0232841) (-5.8,0.0175042) (-5.7,0.0109041) (-5.6,0.00338282) (-5.5,-0.0051673) (-5.4,-0.0148604) (-5.3,-0.0258127) (-5.2,-0.0381391) (-5.1,-0.0519504) (-5.,-0.0673397) (-4.9,-0.0843762) (-4.8,-0.103088) (-4.7,-0.123446) (-4.6,-0.14533) (-4.5,-0.168513) (-4.4,-0.192611) (-4.3,-0.21705) (-4.2,-0.24102) (-4.1,-0.263434) (-4.,-0.282903) (-3.9,-0.297732) (-3.8,-0.305962) (-3.7,-0.305491) (-3.6,-0.294266) (-3.5,-0.270588) (-3.4,-0.23348) (-3.3,-0.183083) (-3.2,-0.120938) (-3.1,-0.0500566) (-3.,0.025324) (-2.9,0.100303) (-2.8,0.170056) (-2.7,0.230558) (-2.6,0.279077) (-2.5,0.314355) (-2.4,0.336486) (-2.3,0.346593) (-2.2,0.346443) (-2.1,0.338081) (-2.,0.323559) (-1.9,0.304759) (-1.8,0.283287) (-1.7,0.260449) (-1.6,0.237258) (-1.5,0.21446) (-1.4,0.192583) (-1.3,0.171972) (-1.2,0.152832) (-1.1,0.135261) (-1.,0.119281) (-0.9,0.104861) (-0.8,0.0919303) (-0.7,0.0803967) (-0.6,0.0701552) (-0.5,0.0610958) (-0.4,0.0531075) (-0.3,0.0460831) (-0.2,0.0399208) (-0.1,0.0345258) (0.,0.0298108) (0.1,0.025696) (0.2,0.0221101) (0.3,0.0189883) (0.4,0.0162733) (0.5,0.0139142) (0.6,0.0118657) (0.7,0.0100882) (0.8,0.00854666) (0.9,0.00721043) (1.,0.00605265) (1.1,0.00504989) (1.2,0.00418167) (1.3,0.00343017) (1.4,0.00277984) (1.5,0.00221721) (1.6,0.00173055) (1.7,0.00130966) (1.8,0.000945713) (1.9,0.000631048) (2.,0.000359024) (2.1,0.000123886) (2.2,-0.0000793498) (2.3,-0.000254996) (2.4,-0.000406788) (2.5,-0.000537956) (2.6,-0.000651296) (2.7,-0.00074923) (2.8,-0.000833846) (2.9,-0.00090695) (3.,-0.000970109) (3.1,-0.00102467) (3.2,-0.00107181) (3.3,-0.00111253) (3.4,-0.00114771) (3.5,-0.0011781) (3.6,-0.00120435) (3.7,-0.00122703) (3.8,-0.00124661) (3.9,-0.00126354) (4.,-0.00127815) (4.1,-0.00129078) (4.2,-0.00130168) (4.3,-0.0013111) (4.4,-0.00131924) (4.5,-0.00132626) (4.6,-0.00133233) (4.7,-0.00133758) (4.8,-0.00134211) (4.9,-0.00134602) (5.,-0.0013494) (5.1,-0.00135231) (5.2,-0.00135484) (5.3,-0.00135701) (5.4,-0.00135889) (5.5,-0.00136052) (5.6,-0.00136192) (5.7,-0.00136313) (5.8,-0.00136418) (5.9,-0.00136508) (6.,-0.00136586) (6.1,-0.00136654) (6.2,-0.00136712) (6.3,-0.00136762) (6.4,-0.00136806) (6.5,-0.00136843) (6.6,-0.00136876) (6.7,-0.00136904) (6.8,-0.00136928) (6.9,-0.00136949) (7.,-0.00136967) (7.1,-0.00136982) (7.2,-0.00136996) (7.3,-0.00137008) (7.4,-0.00137018) (7.5,-0.00137026) (7.6,-0.00137034) (7.7,-0.0013704) (7.8,-0.00137046) (7.9,-0.00137051) (8.,-0.00137055) (8.1,-0.00137059) (8.2,-0.00137062) (8.3,-0.00137064) (8.4,-0.00137067) (8.5,-0.00137069) (8.6,-0.0013707) (8.7,-0.00137072) (8.8,-0.00137073) (8.9,-0.00137074) (9.,-0.00137075) (9.1,-0.00137076) (9.2,-0.00137077) (9.3,-0.00137077) (9.4,-0.00137078) (9.5,-0.00137078) (9.6,-0.00137079) (9.7,-0.00137079) (9.8,-0.00137079) (9.9,-0.0013708) (10.,-0.0013708) 
};

% Final RV 10.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0383823) (-9.9,0.0383675) (-9.8,0.0383505) (-9.7,0.0383306) (-9.6,0.0383082) (-9.5,0.0382814) (-9.4,0.0382511) (-9.3,0.0382156) (-9.2,0.0381747) (-9.1,0.0381272) (-9.,0.0380724) (-8.9,0.0380088) (-8.8,0.0379354) (-8.7,0.0378506) (-8.6,0.0377518) (-8.5,0.0376374) (-8.4,0.0375058) (-8.3,0.0373527) (-8.2,0.0371761) (-8.1,0.0369718) (-8.,0.0367355) (-7.9,0.0364618) (-7.8,0.0361454) (-7.7,0.0357792) (-7.6,0.0353559) (-7.5,0.0348666) (-7.4,0.0343007) (-7.3,0.0336464) (-7.2,0.0328907) (-7.1,0.0320176) (-7.,0.031009) (-6.9,0.0298451) (-6.8,0.0285009) (-6.7,0.0269514) (-6.6,0.025164) (-6.5,0.0231051) (-6.4,0.0207334) (-6.3,0.0180049) (-6.2,0.0148681) (-6.1,0.0112652) (-6.,0.00713202) (-5.9,0.0023969) (-5.8,-0.00301956) (-5.7,-0.00920439) (-5.6,-0.0162516) (-5.5,-0.0242619) (-5.4,-0.0333419) (-5.3,-0.0436) (-5.2,-0.0551431) (-5.1,-0.0680738) (-5.,-0.0824784) (-4.9,-0.09842) (-4.8,-0.115923) (-4.7,-0.134955) (-4.6,-0.155403) (-4.5,-0.177048) (-4.4,-0.199523) (-4.3,-0.222284) (-4.2,-0.244562) (-4.1,-0.265326) (-4.,-0.283261) (-3.9,-0.296765) (-3.8,-0.303982) (-3.7,-0.302927) (-3.6,-0.29166) (-3.5,-0.268576) (-3.4,-0.232759) (-3.3,-0.184345) (-3.2,-0.124799) (-3.1,-0.056976) (-3.,0.0151079) (-2.9,0.08681) (-2.8,0.15356) (-2.7,0.211542) (-2.6,0.258167) (-2.5,0.292238) (-2.4,0.313839) (-2.3,0.32403) (-2.2,0.324476) (-2.1,0.317112) (-2.,0.303879) (-1.9,0.286554) (-1.8,0.26666) (-1.7,0.245435) (-1.6,0.223835) (-1.5,0.202573) (-1.4,0.182148) (-1.3,0.162889) (-1.2,0.144995) (-1.1,0.12856) (-1.,0.113608) (-0.9,0.100111) (-0.8,0.0880045) (-0.7,0.077204) (-0.6,0.0676118) (-0.5,0.0591255) (-0.4,0.0516415) (-0.3,0.0450599) (-0.2,0.0392855) (-0.1,0.0342297) (0.,0.0298108) (0.1,0.0259542) (0.2,0.0225931) (0.3,0.0196669) (0.4,0.0171219) (0.5,0.0149104) (0.6,0.01299) (0.7,0.0113237) (0.8,0.00987848) (0.9,0.00862574) (1.,0.00754028) (1.1,0.00660013) (1.2,0.00578612) (1.3,0.00508153) (1.4,0.00447179) (1.5,0.00394426) (1.6,0.00348797) (1.7,0.00309333) (1.8,0.00275209) (1.9,0.00245705) (2.,0.00220199) (2.1,0.00198151) (2.2,0.00179095) (2.3,0.00162625) (2.4,0.00148393) (2.5,0.00136094) (2.6,0.00125466) (2.7,0.00116284) (2.8,0.00108349) (2.9,0.00101495) (3.,0.000955725) (3.1,0.000904561) (3.2,0.000860361) (3.3,0.000822179) (3.4,0.000789193) (3.5,0.0007607) (3.6,0.000736082) (3.7,0.000714821) (3.8,0.000696453) (3.9,0.000680587) (4.,0.000666885) (4.1,0.000655046) (4.2,0.000644821) (4.3,0.000635988) (4.4,0.000628361) (4.5,0.000621772) (4.6,0.000616078) (4.7,0.000611161) (4.8,0.000606915) (4.9,0.000603248) (5.,0.000600081) (5.1,0.000597341) (5.2,0.000594979) (5.3,0.000592938) (5.4,0.000591172) (5.5,0.000589652) (5.6,0.000588336) (5.7,0.000587198) (5.8,0.000586216) (5.9,0.00058537) (6.,0.000584637) (6.1,0.000584005) (6.2,0.000583459) (6.3,0.000582986) (6.4,0.000582578) (6.5,0.000582228) (6.6,0.000581922) (6.7,0.000581659) (6.8,0.000581434) (6.9,0.000581237) (7.,0.00058107) (7.1,0.000580923) (7.2,0.000580797) (7.3,0.000580688) (7.4,0.000580592) (7.5,0.000580512) (7.6,0.000580442) (7.7,0.00058038) (7.8,0.000580329) (7.9,0.000580281) (8.,0.000580243) (8.1,0.000580209) (8.2,0.00058018) (8.3,0.000580156) (8.4,0.000580132) (8.5,0.000580115) (8.6,0.000580098) (8.7,0.000580084) (8.8,0.000580072) (8.9,0.000580061) (9.,0.000580054) (9.1,0.000580045) (9.2,0.000580039) (9.3,0.000580032) (9.4,0.000580029) (9.5,0.000580023) (9.6,0.000580019) (9.7,0.000580018) (9.8,0.000580015) (9.9,0.000580011) (10.,0.000580008) 
};













% Start of data.

% Final RV 1.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.124996) (-9.9,0.124982) (-9.8,0.124965) (-9.7,0.124945) (-9.6,0.124923) (-9.5,0.124896) (-9.4,0.124866) (-9.3,0.124831) (-9.2,0.124791) (-9.1,0.124744) (-9.,0.12469) (-8.9,0.124627) (-8.8,0.124554) (-8.7,0.12447) (-8.6,0.124372) (-8.5,0.124259) (-8.4,0.124129) (-8.3,0.123977) (-8.2,0.123803) (-8.1,0.1236) (-8.,0.123366) (-7.9,0.123095) (-7.8,0.122782) (-7.7,0.12242) (-7.6,0.122001) (-7.5,0.121516) (-7.4,0.120956) (-7.3,0.120309) (-7.2,0.119561) (-7.1,0.118696) (-7.,0.117698) (-6.9,0.116546) (-6.8,0.115214) (-6.7,0.11368) (-6.6,0.11191) (-6.5,0.109871) (-6.4,0.107521) (-6.3,0.104817) (-6.2,0.101709) (-6.1,0.0981384) (-6.,0.094041) (-5.9,0.0893457) (-5.8,0.0839731) (-5.7,0.0778367) (-5.6,0.0708419) (-5.5,0.0628874) (-5.4,0.0538659) (-5.3,0.0436679) (-5.2,0.032184) (-5.1,0.0193084) (-5.,0.00495041) (-4.9,-0.0109595) (-4.8,-0.0284547) (-4.7,-0.0475155) (-4.6,-0.0680444) (-4.5,-0.0898428) (-4.4,-0.112574) (-4.3,-0.135727) (-4.2,-0.15858) (-4.1,-0.180156) (-4.,-0.199206) (-3.9,-0.214203) (-3.8,-0.223379) (-3.7,-0.224831) (-3.6,-0.216701) (-3.5,-0.197442) (-3.4,-0.166161) (-3.3,-0.122967) (-3.2,-0.0692306) (-3.1,-0.00764863) (-3.,0.0579772) (-2.9,0.123247) (-2.8,0.183828) (-2.7,0.236111) (-2.6,0.27765) (-2.5,0.307327) (-2.4,0.325244) (-2.3,0.332426) (-2.2,0.330478) (-2.1,0.32125) (-2.,0.306597) (-1.9,0.288215) (-1.8,0.267553) (-1.7,0.245783) (-1.6,0.223812) (-1.5,0.202307) (-1.4,0.181736) (-1.3,0.1624) (-1.2,0.144478) (-1.1,0.128049) (-1.,0.113126) (-0.9,0.0996714) (-0.8,0.087616) (-0.7,0.0768705) (-0.6,0.0673338) (-0.5,0.058902) (-0.4,0.05147) (-0.3,0.0449369) (-0.2,0.0392075) (-0.1,0.0341926) (0.,0.0298108) (0.1,0.0259875) (0.2,0.0226562) (0.3,0.0197565) (0.4,0.017235) (0.5,0.0150441) (0.6,0.013142) (0.7,0.0114917) (0.8,0.0100605) (0.9,0.00882005) (1.,0.0077453) (1.1,0.0068145) (1.2,0.00600864) (1.3,0.00531113) (1.4,0.00470755) (1.5,0.00418537) (1.6,0.00373373) (1.7,0.00334312) (1.8,0.00300537) (1.9,0.00271336) (2.,0.00246093) (2.1,0.00224273) (2.2,0.00205414) (2.3,0.00189114) (2.4,0.0017503) (2.5,0.00162858) (2.6,0.00152341) (2.7,0.00143254) (2.8,0.00135402) (2.9,0.00128619) (3.,0.00122758) (3.1,0.00117696) (3.2,0.00113322) (3.3,0.00109543) (3.4,0.00106279) (3.5,0.00103459) (3.6,0.00101024) (3.7,0.000989194) (3.8,0.00097102) (3.9,0.00095532) (4.,0.000941762) (4.1,0.000930046) (4.2,0.000919927) (4.3,0.000911188) (4.4,0.00090364) (4.5,0.000897119) (4.6,0.000891485) (4.7,0.00088662) (4.8,0.000882418) (4.9,0.00087879) (5.,0.000875655) (5.1,0.000872945) (5.2,0.000870608) (5.3,0.000868588) (5.4,0.000866841) (5.5,0.000865337) (5.6,0.000864034) (5.7,0.000862908) (5.8,0.000861936) (5.9,0.000861099) (6.,0.000860374) (6.1,0.000859748) (6.2,0.000859208) (6.3,0.000858741) (6.4,0.000858337) (6.5,0.00085799) (6.6,0.000857687) (6.7,0.000857428) (6.8,0.000857205) (6.9,0.00085701) (7.,0.000856845) (7.1,0.0008567) (7.2,0.000856575) (7.3,0.000856466) (7.4,0.000856371) (7.5,0.000856293) (7.6,0.000856223) (7.7,0.000856162) (7.8,0.000856111) (7.9,0.000856064) (8.,0.000856026) (8.1,0.000855992) (8.2,0.000855964) (8.3,0.00085594) (8.4,0.000855917) (8.5,0.0008559) (8.6,0.000855883) (8.7,0.000855868) (8.8,0.000855856) (8.9,0.000855845) (9.,0.000855839) (9.1,0.000855831) (9.2,0.000855825) (9.3,0.000855817) (9.4,0.000855815) (9.5,0.000855808) (9.6,0.000855805) (9.7,0.000855803) (9.8,0.0008558) (9.9,0.000855795) (10.,0.000855794) 
};

% Final RV 2.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,-0.217653) (-9.9,-0.217666) (-9.8,-0.217684) (-9.7,-0.217704) (-9.6,-0.217725) (-9.5,-0.217751) (-9.4,-0.217781) (-9.3,-0.217816) (-9.2,-0.217856) (-9.1,-0.217903) (-9.,-0.217956) (-8.9,-0.218018) (-8.8,-0.21809) (-8.7,-0.218174) (-8.6,-0.218271) (-8.5,-0.218383) (-8.4,-0.218511) (-8.3,-0.218662) (-8.2,-0.218834) (-8.1,-0.219034) (-8.,-0.219267) (-7.9,-0.219535) (-7.8,-0.219845) (-7.7,-0.220205) (-7.6,-0.220619) (-7.5,-0.221098) (-7.4,-0.221652) (-7.3,-0.222293) (-7.2,-0.223032) (-7.1,-0.223887) (-7.,-0.224874) (-6.9,-0.226013) (-6.8,-0.227328) (-6.7,-0.228845) (-6.6,-0.230593) (-6.5,-0.232604) (-6.4,-0.234922) (-6.3,-0.237588) (-6.2,-0.24065) (-6.1,-0.244166) (-6.,-0.248196) (-5.9,-0.25281) (-5.8,-0.258081) (-5.7,-0.264097) (-5.6,-0.270943) (-5.5,-0.278713) (-5.4,-0.287507) (-5.3,-0.297424) (-5.2,-0.308558) (-5.1,-0.321) (-5.,-0.334814) (-4.9,-0.350044) (-4.8,-0.366684) (-4.7,-0.384672) (-4.6,-0.40385) (-4.5,-0.423945) (-4.4,-0.44453) (-4.3,-0.464982) (-4.2,-0.48444) (-4.1,-0.501761) (-4.,-0.5155) (-3.9,-0.523912) (-3.8,-0.524988) (-3.7,-0.516586) (-3.6,-0.496632) (-3.5,-0.463427) (-3.4,-0.41603) (-3.3,-0.354658) (-3.2,-0.280974) (-3.1,-0.19816) (-3.,-0.11066) (-2.9,-0.0235959) (-2.8,0.057985) (-2.7,0.129859) (-2.6,0.189139) (-2.5,0.234455) (-2.4,0.265839) (-2.3,0.28439) (-2.2,0.291883) (-2.1,0.290392) (-2.,0.282016) (-1.9,0.268685) (-1.8,0.252065) (-1.7,0.233516) (-1.6,0.214104) (-1.5,0.19463) (-1.4,0.175669) (-1.3,0.157611) (-1.2,0.140703) (-1.1,0.12508) (-1.,0.110799) (-0.9,0.0978569) (-0.8,0.0862115) (-0.7,0.0757948) (-0.6,0.0665227) (-0.5,0.0583043) (-0.4,0.0510451) (-0.3,0.0446524) (-0.2,0.0390373) (-0.1,0.0341159) (0.,0.0298108) (0.1,0.0260506) (0.2,0.0227714) (0.3,0.0199148) (0.4,0.0174291) (0.5,0.0152682) (0.6,0.0133911) (0.7,0.0117616) (0.8,0.010348) (0.9,0.00912234) (1.,0.00806007) (1.1,0.00713983) (1.2,0.0063429) (1.3,0.00565299) (1.4,0.00505586) (1.5,0.00453918) (1.6,0.00409222) (1.7,0.00370562) (1.8,0.00337129) (1.9,0.0030822) (2.,0.00283229) (2.1,0.00261622) (2.2,0.00242948) (2.3,0.00226807) (2.4,0.00212859) (2.5,0.00200804) (2.6,0.00190388) (2.7,0.00181386) (2.8,0.0017361) (2.9,0.0016689) (3.,0.00161085) (3.1,0.0015607) (3.2,0.00151737) (3.3,0.00147993) (3.4,0.00144759) (3.5,0.00141966) (3.6,0.00139554) (3.7,0.00137468) (3.8,0.00135669) (3.9,0.00134113) (4.,0.0013277) (4.1,0.00131609) (4.2,0.00130606) (4.3,0.00129741) (4.4,0.00128992) (4.5,0.00128346) (4.6,0.00127789) (4.7,0.00127307) (4.8,0.0012689) (4.9,0.00126531) (5.,0.00126219) (5.1,0.00125951) (5.2,0.0012572) (5.3,0.0012552) (5.4,0.00125347) (5.5,0.00125197) (5.6,0.00125068) (5.7,0.00124957) (5.8,0.00124861) (5.9,0.00124778) (6.,0.00124706) (6.1,0.00124644) (6.2,0.0012459) (6.3,0.00124544) (6.4,0.00124504) (6.5,0.00124469) (6.6,0.00124439) (6.7,0.00124414) (6.8,0.00124391) (6.9,0.00124373) (7.,0.00124356) (7.1,0.00124342) (7.2,0.00124329) (7.3,0.00124318) (7.4,0.0012431) (7.5,0.00124301) (7.6,0.00124295) (7.7,0.00124288) (7.8,0.00124283) (7.9,0.00124279) (8.,0.00124275) (8.1,0.00124272) (8.2,0.00124269) (8.3,0.00124267) (8.4,0.00124264) (8.5,0.00124262) (8.6,0.00124261) (8.7,0.00124259) (8.8,0.00124259) (8.9,0.00124257) (9.,0.00124257) (9.1,0.00124256) (9.2,0.00124255) (9.3,0.00124254) (9.4,0.00124254) (9.5,0.00124254) (9.6,0.00124254) (9.7,0.00124253) (9.8,0.00124253) (9.9,0.00124252) (10.,0.00124252) 
};

% Final RV 3.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0952505) (-9.9,0.0952353) (-9.8,0.0952175) (-9.7,0.0951967) (-9.6,0.0951735) (-9.5,0.0951462) (-9.4,0.0951142) (-9.3,0.0950779) (-9.2,0.0950351) (-9.1,0.0949858) (-9.,0.0949293) (-8.9,0.0948632) (-8.8,0.0947867) (-8.7,0.0946987) (-8.6,0.0945963) (-8.5,0.0944776) (-8.4,0.0943413) (-8.3,0.0941818) (-8.2,0.093999) (-8.1,0.093787) (-8.,0.0935411) (-7.9,0.0932573) (-7.8,0.0929285) (-7.7,0.0925486) (-7.6,0.0921092) (-7.5,0.0916013) (-7.4,0.0910138) (-7.3,0.0903349) (-7.2,0.0895509) (-7.1,0.0886442) (-7.,0.0875974) (-6.9,0.0863892) (-6.8,0.0849933) (-6.7,0.0833845) (-6.6,0.0815283) (-6.5,0.0793908) (-6.4,0.0769277) (-6.3,0.0740935) (-6.2,0.0708356) (-6.1,0.0670928) (-6.,0.0627985) (-5.9,0.0578779) (-5.8,0.0522485) (-5.7,0.0458196) (-5.6,0.0384921) (-5.5,0.0301606) (-5.4,0.0207133) (-5.3,0.010037) (-5.2,-0.00198253) (-5.1,-0.0154541) (-5.,-0.0304712) (-4.9,-0.0471033) (-4.8,-0.065382) (-4.7,-0.0852821) (-4.6,-0.106695) (-4.5,-0.129406) (-4.4,-0.153051) (-4.3,-0.177083) (-4.2,-0.200729) (-4.1,-0.22295) (-4.,-0.242413) (-3.9,-0.257492) (-3.8,-0.266309) (-3.7,-0.266842) (-3.6,-0.257118) (-3.5,-0.235499) (-3.4,-0.201042) (-3.3,-0.153872) (-3.2,-0.0954577) (-3.1,-0.028679) (-3.,0.0424094) (-2.9,0.113116) (-2.8,0.178821) (-2.7,0.235673) (-2.6,0.281062) (-2.5,0.313787) (-2.4,0.333949) (-2.3,0.342633) (-2.2,0.341537) (-2.1,0.33263) (-2.,0.317879) (-1.9,0.299092) (-1.8,0.27781) (-1.7,0.255283) (-1.6,0.232477) (-1.5,0.210108) (-1.4,0.188676) (-1.3,0.168508) (-1.2,0.149797) (-1.1,0.132633) (-1.,0.117032) (-0.9,0.102961) (-0.8,0.0903476) (-0.7,0.079101) (-0.6,0.0691171) (-0.5,0.0602877) (-0.4,0.0525036) (-0.3,0.0456601) (-0.2,0.0396574) (-0.1,0.0344027) (0.,0.0298108) (0.1,0.0258039) (0.2,0.0223122) (0.3,0.0192727) (0.4,0.0166295) (0.5,0.0143328) (0.6,0.0123387) (0.7,0.0106084) (0.8,0.00910788) (0.9,0.00780725) (1.,0.00668034) (1.1,0.00570434) (1.2,0.00485932) (1.3,0.00412792) (1.4,0.00349498) (1.5,0.00294742) (1.6,0.00247379) (1.7,0.00206418) (1.8,0.00170999) (1.9,0.00140376) (2.,0.00113903) (2.1,0.000910207) (2.2,0.000712425) (2.3,0.000541495) (2.4,0.000393778) (2.5,0.000266132) (2.6,0.000155836) (2.7,0.0000605347) (2.8,-0.000021809) (2.9,-0.0000929497) (3.,-0.00015441) (3.1,-0.000207509) (3.2,-0.00025338) (3.3,-0.000293005) (3.4,-0.000327239) (3.5,-0.000356809) (3.6,-0.000382358) (3.7,-0.000404422) (3.8,-0.000423484) (3.9,-0.000439951) (4.,-0.000454168) (4.1,-0.000466456) (4.2,-0.000477069) (4.3,-0.000486234) (4.4,-0.000494149) (4.5,-0.000500989) (4.6,-0.000506899) (4.7,-0.000512001) (4.8,-0.000516408) (4.9,-0.000520212) (5.,-0.000523499) (5.1,-0.000526343) (5.2,-0.000528793) (5.3,-0.000530911) (5.4,-0.000532745) (5.5,-0.000534321) (5.6,-0.000535687) (5.7,-0.000536869) (5.8,-0.000537888) (5.9,-0.000538765) (6.,-0.000539526) (6.1,-0.000540182) (6.2,-0.000540749) (6.3,-0.000541239) (6.4,-0.000541662) (6.5,-0.000542026) (6.6,-0.000542345) (6.7,-0.000542616) (6.8,-0.00054285) (6.9,-0.000543054) (7.,-0.000543227) (7.1,-0.000543379) (7.2,-0.000543509) (7.3,-0.000543625) (7.4,-0.000543724) (7.5,-0.000543805) (7.6,-0.00054388) (7.7,-0.000543944) (7.8,-0.000543997) (7.9,-0.000544047) (8.,-0.000544086) (8.1,-0.000544123) (8.2,-0.000544151) (8.3,-0.000544176) (8.4,-0.000544202) (8.5,-0.000544218) (8.6,-0.000544237) (8.7,-0.000544252) (8.8,-0.000544265) (8.9,-0.000544277) (9.,-0.000544281) (9.1,-0.000544291) (9.2,-0.000544296) (9.3,-0.000544305) (9.4,-0.000544307) (9.5,-0.000544316) (9.6,-0.000544317) (9.7,-0.00054432) (9.8,-0.000544322) (9.9,-0.00054433) (10.,-0.000544331) 
};

% Final RV 4.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,-0.00976013) (-9.9,-0.00977537) (-9.8,-0.00979251) (-9.7,-0.00981291) (-9.6,-0.00983574) (-9.5,-0.00986304) (-9.4,-0.00989389) (-9.3,-0.00992985) (-9.2,-0.00997174) (-9.1,-0.0100202) (-9.,-0.0100759) (-8.9,-0.0101406) (-8.8,-0.0102157) (-8.7,-0.010302) (-8.6,-0.0104026) (-8.5,-0.0105192) (-8.4,-0.0106533) (-8.3,-0.0108093) (-8.2,-0.0109891) (-8.1,-0.0111975) (-8.,-0.0114384) (-7.9,-0.0117171) (-7.8,-0.0120396) (-7.7,-0.0124125) (-7.6,-0.012844) (-7.5,-0.0133426) (-7.4,-0.0139192) (-7.3,-0.0145855) (-7.2,-0.0153555) (-7.1,-0.016245) (-7.,-0.0172725) (-6.9,-0.0184582) (-6.8,-0.0198275) (-6.7,-0.0214057) (-6.6,-0.0232264) (-6.5,-0.0253233) (-6.4,-0.0277387) (-6.3,-0.0305172) (-6.2,-0.0337111) (-6.1,-0.0373794) (-6.,-0.0415871) (-5.9,-0.0464069) (-5.8,-0.0519195) (-5.7,-0.0582126) (-5.6,-0.0653818) (-5.5,-0.073529) (-5.4,-0.0827616) (-5.3,-0.0931883) (-5.2,-0.104917) (-5.1,-0.118049) (-5.,-0.132669) (-4.9,-0.148839) (-4.8,-0.166576) (-4.7,-0.185844) (-4.6,-0.206517) (-4.5,-0.228361) (-4.4,-0.25099) (-4.3,-0.273832) (-4.2,-0.296084) (-4.1,-0.31667) (-4.,-0.334221) (-3.9,-0.34707) (-3.8,-0.353292) (-3.7,-0.350826) (-3.6,-0.337663) (-3.5,-0.312144) (-3.4,-0.273326) (-3.3,-0.221365) (-3.2,-0.157797) (-3.1,-0.0856029) (-3.,-0.00897014) (-2.9,0.0672617) (-2.8,0.138328) (-2.7,0.200251) (-2.6,0.250325) (-2.5,0.287293) (-2.4,0.311232) (-2.3,0.323232) (-2.2,0.325019) (-2.1,0.318597) (-2.,0.30598) (-1.9,0.289015) (-1.8,0.269288) (-1.7,0.248085) (-1.6,0.226407) (-1.5,0.204999) (-1.4,0.184387) (-1.3,0.164917) (-1.2,0.146802) (-1.1,0.130147) (-1.,0.114982) (-0.9,0.101283) (-0.8,0.0889885) (-0.7,0.078015) (-0.6,0.0682652) (-0.5,0.0596367) (-0.4,0.052025) (-0.3,0.0453295) (-0.2,0.039454) (-0.1,0.0343086) (0.,0.0298108) (0.1,0.0258848) (0.2,0.0224627) (0.3,0.0194831) (0.4,0.0168915) (0.5,0.0146393) (0.6,0.0126835) (0.7,0.0109862) (0.8,0.00951415) (0.9,0.00823805) (1.,0.00713229) (1.1,0.00617454) (1.2,0.00534526) (1.3,0.00462742) (1.4,0.0040062) (1.5,0.00346874) (1.6,0.00300384) (1.7,0.00260175) (1.8,0.00225405) (1.9,0.00195344) (2.,0.00169355) (2.1,0.0014689) (2.2,0.00127473) (2.3,0.00110691) (2.4,0.000961881) (2.5,0.000836557) (2.6,0.000728265) (2.7,0.000634694) (2.8,0.000553846) (2.9,0.000483996) (3.,0.00042365) (3.1,0.000371514) (3.2,0.000326474) (3.3,0.000287564) (3.4,0.000253953) (3.5,0.000224917) (3.6,0.000199833) (3.7,0.000178165) (3.8,0.00015945) (3.9,0.000143283) (4.,0.000129318) (4.1,0.000117255) (4.2,0.000106836) (4.3,0.0000978348) (4.4,0.0000900608) (4.5,0.0000833475) (4.6,0.0000775465) (4.7,0.0000725365) (4.8,0.0000682087) (4.9,0.0000644712) (5.,0.000061243) (5.1,0.0000584536) (5.2,0.0000560451) (5.3,0.0000539647) (5.4,0.0000521676) (5.5,0.0000506164) (5.6,0.0000492751) (5.7,0.0000481175) (5.8,0.0000471166) (5.9,0.0000462531) (6.,0.0000455068) (6.1,0.0000448621) (6.2,0.0000443054) (6.3,0.0000438241) (6.4,0.000043409) (6.5,0.000043052) (6.6,0.0000427415) (6.7,0.0000424728) (6.8,0.0000422426) (6.9,0.0000420419) (7.,0.00004187) (7.1,0.0000417216) (7.2,0.0000415916) (7.3,0.0000414818) (7.4,0.0000413849) (7.5,0.0000413018) (7.6,0.0000412308) (7.7,0.0000411687) (7.8,0.0000411167) (7.9,0.0000410688) (8.,0.0000410288) (8.1,0.0000409954) (8.2,0.0000409653) (8.3,0.0000409401) (8.4,0.0000409171) (8.5,0.0000408978) (8.6,0.0000408824) (8.7,0.0000408686) (8.8,0.0000408555) (8.9,0.0000408448) (9.,0.0000408361) (9.1,0.0000408266) (9.2,0.0000408201) (9.3,0.0000408137) (9.4,0.0000408092) (9.5,0.0000408054) (9.6,0.0000408008) (9.7,0.0000407986) (9.8,0.0000407947) (9.9,0.0000407937) (10.,0.0000407896) 
};

% Final RV 5.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.133482) (-9.9,0.133468) (-9.8,0.13345) (-9.7,0.133429) (-9.6,0.133406) (-9.5,0.13338) (-9.4,0.133348) (-9.3,0.133312) (-9.2,0.13327) (-9.1,0.133222) (-9.,0.133166) (-8.9,0.133101) (-8.8,0.133026) (-8.7,0.132939) (-8.6,0.132838) (-8.5,0.132721) (-8.4,0.132587) (-8.3,0.132429) (-8.2,0.132249) (-8.1,0.13204) (-8.,0.131798) (-7.9,0.131518) (-7.8,0.131194) (-7.7,0.13082) (-7.6,0.130387) (-7.5,0.129886) (-7.4,0.129307) (-7.3,0.128638) (-7.2,0.127866) (-7.1,0.126972) (-7.,0.12594) (-6.9,0.124749) (-6.8,0.123374) (-6.7,0.121787) (-6.6,0.119958) (-6.5,0.117851) (-6.4,0.115422) (-6.3,0.112628) (-6.2,0.109416) (-6.1,0.105725) (-6.,0.10149) (-5.9,0.0966371) (-5.8,0.0910843) (-5.7,0.0847414) (-5.6,0.0775113) (-5.5,0.0692893) (-5.4,0.0599637) (-5.3,0.0494217) (-5.2,0.03755) (-5.1,0.0242389) (-5.,0.00939432) (-4.9,-0.00705602) (-4.8,-0.0251471) (-4.7,-0.0448594) (-4.6,-0.0660928) (-4.5,-0.0886437) (-4.4,-0.112165) (-4.3,-0.136131) (-4.2,-0.159797) (-4.1,-0.182158) (-4.,-0.201926) (-3.9,-0.217524) (-3.8,-0.227131) (-3.7,-0.228784) (-3.6,-0.220567) (-3.5,-0.200883) (-3.4,-0.168811) (-3.3,-0.12446) (-3.2,-0.0692435) (-3.1,-0.00594014) (-3.,0.0615318) (-2.9,0.128637) (-2.8,0.19091) (-2.7,0.24463) (-2.6,0.287277) (-2.5,0.3177) (-2.4,0.336004) (-2.3,0.343249) (-2.2,0.341089) (-2.1,0.331434) (-2.,0.316195) (-1.9,0.297123) (-1.8,0.27571) (-1.7,0.253166) (-1.6,0.230424) (-1.5,0.208171) (-1.4,0.18689) (-1.3,0.16689) (-1.2,0.148355) (-1.1,0.131367) (-1.,0.115936) (-0.9,0.102026) (-0.8,0.0895629) (-0.7,0.0784543) (-0.6,0.068596) (-0.5,0.0598801) (-0.4,0.0521978) (-0.3,0.0454451) (-0.2,0.039523) (-0.1,0.0343397) (0.,0.0298108) (0.1,0.0258592) (0.2,0.0224161) (0.3,0.0194192) (0.4,0.0168131) (0.5,0.0145489) (0.6,0.0125831) (0.7,0.0108774) (0.8,0.00939833) (0.9,0.00811632) (1.,0.00700559) (1.1,0.00604363) (1.2,0.00521079) (1.3,0.00448993) (1.4,0.00386615) (1.5,0.00332651) (1.6,0.00285974) (1.7,0.00245607) (1.8,0.00210702) (1.9,0.00180524) (2.,0.00154436) (2.1,0.00131886) (2.2,0.00112396) (2.3,0.000955518) (2.4,0.000809953) (2.5,0.000684167) (2.6,0.000575479) (2.7,0.000481567) (2.8,0.000400425) (2.9,0.000330322) (3.,0.000269758) (3.1,0.000217434) (3.2,0.000172233) (3.3,0.000133184) (3.4,0.0000994521) (3.5,0.0000703121) (3.6,0.0000451393) (3.7,0.0000233947) (3.8,0.00000461255) (3.9,-0.0000116116) (4.,-0.0000256262) (4.1,-0.0000377319) (4.2,-0.0000481883) (4.3,-0.0000572209) (4.4,-0.0000650224) (4.5,-0.00007176) (4.6,-0.000077581) (4.7,-0.0000826087) (4.8,-0.0000869518) (4.9,-0.0000907024) (5.,-0.0000939422) (5.1,-0.0000967411) (5.2,-0.0000991581) (5.3,-0.000101246) (5.4,-0.000103049) (5.5,-0.000104606) (5.6,-0.000105952) (5.7,-0.000107114) (5.8,-0.000108118) (5.9,-0.000108985) (6.,-0.000109734) (6.1,-0.000110381) (6.2,-0.000110939) (6.3,-0.000111422) (6.4,-0.000111839) (6.5,-0.000112197) (6.6,-0.000112509) (6.7,-0.000112778) (6.8,-0.000113009) (6.9,-0.00011321) (7.,-0.000113383) (7.1,-0.000113532) (7.2,-0.000113662) (7.3,-0.000113773) (7.4,-0.00011387) (7.5,-0.000113953) (7.6,-0.000114025) (7.7,-0.000114087) (7.8,-0.00011414) (7.9,-0.000114187) (8.,-0.000114227) (8.1,-0.000114261) (8.2,-0.000114291) (8.3,-0.000114316) (8.4,-0.000114339) (8.5,-0.000114359) (8.6,-0.000114374) (8.7,-0.000114389) (8.8,-0.000114402) (8.9,-0.000114412) (9.,-0.000114422) (9.1,-0.00011443) (9.2,-0.000114437) (9.3,-0.000114443) (9.4,-0.000114447) (9.5,-0.000114452) (9.6,-0.000114456) (9.7,-0.000114459) (9.8,-0.000114462) (9.9,-0.000114464) (10.,-0.000114467) 
};

% Final RV 6.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0136137) (-9.9,0.013598) (-9.8,0.0135804) (-9.7,0.0135596) (-9.6,0.0135361) (-9.5,0.013508) (-9.4,0.0134764) (-9.3,0.0134396) (-9.2,0.0133966) (-9.1,0.0133469) (-9.,0.0132898) (-8.9,0.0132234) (-8.8,0.0131463) (-8.7,0.0130578) (-8.6,0.0129546) (-8.5,0.0128351) (-8.4,0.0126975) (-8.3,0.0125376) (-8.2,0.012353) (-8.1,0.0121392) (-8.,0.0118922) (-7.9,0.0116063) (-7.8,0.0112755) (-7.7,0.010893) (-7.6,0.0104503) (-7.5,0.00993895) (-7.4,0.0093475) (-7.3,0.00866394) (-7.2,0.00787403) (-7.1,0.00696152) (-7.,0.00590741) (-6.9,0.00469113) (-6.8,0.00328629) (-6.7,0.00166721) (-6.6,-0.000200695) (-6.5,-0.00235212) (-6.4,-0.00483029) (-6.3,-0.00768123) (-6.2,-0.0109586) (-6.1,-0.0147227) (-6.,-0.0190407) (-5.9,-0.0239872) (-5.8,-0.029645) (-5.7,-0.0361047) (-5.6,-0.0434643) (-5.5,-0.0518289) (-5.4,-0.061309) (-5.3,-0.0720171) (-5.2,-0.0840644) (-5.1,-0.0975568) (-5.,-0.112583) (-4.9,-0.129206) (-4.8,-0.147449) (-4.7,-0.167276) (-4.6,-0.188563) (-4.5,-0.211076) (-4.4,-0.234426) (-4.3,-0.258032) (-4.2,-0.281084) (-4.1,-0.302489) (-4.,-0.320857) (-3.9,-0.334497) (-3.8,-0.341451) (-3.7,-0.339623) (-3.6,-0.326971) (-3.5,-0.301804) (-3.4,-0.263159) (-3.3,-0.211188) (-3.2,-0.147444) (-3.1,-0.0749494) (-3.,0.00204933) (-2.9,0.0786429) (-2.8,0.149998) (-2.7,0.21208) (-2.6,0.262148) (-2.5,0.298931) (-2.4,0.322513) (-2.3,0.334006) (-2.2,0.335166) (-2.1,0.328033) (-2.,0.314652) (-1.9,0.296904) (-1.8,0.276394) (-1.7,0.25443) (-1.6,0.232028) (-1.5,0.209938) (-1.4,0.188694) (-1.3,0.168646) (-1.2,0.150005) (-1.1,0.132874) (-1.,0.117283) (-0.9,0.103204) (-0.8,0.0905722) (-0.7,0.0793003) (-0.6,0.0692872) (-0.5,0.0604271) (-0.4,0.0526123) (-0.3,0.0457389) (-0.2,0.0397079) (-0.1,0.0344269) (0.,0.0298108) (0.1,0.0257818) (0.2,0.0222703) (0.3,0.0192129) (0.4,0.0165538) (0.5,0.0142429) (0.6,0.0122363) (0.7,0.010495) (0.8,0.00898476) (0.9,0.00767561) (1.,0.00654124) (1.1,0.00555872) (1.2,0.00470801) (1.3,0.00397163) (1.4,0.00333438) (1.5,0.00278305) (1.6,0.00230615) (1.7,0.0018937) (1.8,0.00153704) (1.9,0.00122867) (2.,0.000962093) (2.1,0.000731657) (2.2,0.000532483) (2.3,0.000360346) (2.4,0.000211586) (2.5,0.0000830355) (2.6,-0.0000280429) (2.7,-0.000124021) (2.8,-0.00020695) (2.9,-0.000278597) (3.,-0.000340495) (3.1,-0.000393973) (3.2,-0.000440171) (3.3,-0.000480079) (3.4,-0.000514558) (3.5,-0.000544339) (3.6,-0.00057007) (3.7,-0.000592292) (3.8,-0.000611491) (3.9,-0.000628076) (4.,-0.000642395) (4.1,-0.000654771) (4.2,-0.00066546) (4.3,-0.00067469) (4.4,-0.000682663) (4.5,-0.000689551) (4.6,-0.000695502) (4.7,-0.000700641) (4.8,-0.00070508) (4.9,-0.000708911) (5.,-0.000712224) (5.1,-0.000715086) (5.2,-0.000717554) (5.3,-0.000719687) (5.4,-0.000721533) (5.5,-0.000723123) (5.6,-0.000724499) (5.7,-0.000725688) (5.8,-0.000726714) (5.9,-0.000727598) (6.,-0.000728364) (6.1,-0.000729024) (6.2,-0.000729596) (6.3,-0.000730089) (6.4,-0.000730515) (6.5,-0.000730883) (6.6,-0.000731203) (6.7,-0.000731475) (6.8,-0.000731713) (6.9,-0.000731916) (7.,-0.000732091) (7.1,-0.000732245) (7.2,-0.000732376) (7.3,-0.000732494) (7.4,-0.000732591) (7.5,-0.000732675) (7.6,-0.000732749) (7.7,-0.000732814) (7.8,-0.000732867) (7.9,-0.000732916) (8.,-0.000732956) (8.1,-0.000732994) (8.2,-0.000733022) (8.3,-0.000733048) (8.4,-0.000733073) (8.5,-0.00073309) (8.6,-0.000733108) (8.7,-0.000733124) (8.8,-0.000733136) (8.9,-0.000733148) (9.,-0.000733154) (9.1,-0.000733162) (9.2,-0.000733169) (9.3,-0.000733177) (9.4,-0.00073318) (9.5,-0.000733187) (9.6,-0.000733189) (9.7,-0.000733193) (9.8,-0.000733195) (9.9,-0.000733201) (10.,-0.000733202) 
};

% Final RV 7.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,-0.0206157) (-9.9,-0.020631) (-9.8,-0.0206486) (-9.7,-0.0206693) (-9.6,-0.0206924) (-9.5,-0.0207201) (-9.4,-0.0207515) (-9.3,-0.0207882) (-9.2,-0.0208305) (-9.1,-0.0208798) (-9.,-0.0209365) (-8.9,-0.0210023) (-8.8,-0.0210784) (-8.7,-0.0211661) (-8.6,-0.0212684) (-8.5,-0.0213868) (-8.4,-0.0215231) (-8.3,-0.0216815) (-8.2,-0.0218644) (-8.1,-0.0220759) (-8.,-0.0223205) (-7.9,-0.0226038) (-7.8,-0.0229314) (-7.7,-0.0233104) (-7.6,-0.0237486) (-7.5,-0.024255) (-7.4,-0.0248408) (-7.3,-0.025518) (-7.2,-0.0263003) (-7.1,-0.0272039) (-7.,-0.0282477) (-6.9,-0.0294522) (-6.8,-0.0308432) (-6.7,-0.0324466) (-6.6,-0.0342961) (-6.5,-0.0364262) (-6.4,-0.03888) (-6.3,-0.0417023) (-6.2,-0.0449468) (-6.1,-0.0486729) (-6.,-0.0529469) (-5.9,-0.0578425) (-5.8,-0.0634417) (-5.7,-0.0698333) (-5.6,-0.0771144) (-5.5,-0.0853884) (-5.4,-0.0947643) (-5.3,-0.105352) (-5.2,-0.11726) (-5.1,-0.130593) (-5.,-0.145434) (-4.9,-0.161845) (-4.8,-0.179846) (-4.7,-0.199394) (-4.6,-0.220362) (-4.5,-0.242511) (-4.4,-0.265443) (-4.3,-0.288575) (-4.2,-0.311087) (-4.1,-0.331881) (-4.,-0.349558) (-3.9,-0.362419) (-3.8,-0.368501) (-3.7,-0.365701) (-3.6,-0.351972) (-3.5,-0.325623) (-3.4,-0.285694) (-3.3,-0.232349) (-3.2,-0.167154) (-3.1,-0.0931551) (-3.,-0.0146261) (-2.9,0.0634928) (-2.8,0.136339) (-2.7,0.199851) (-2.6,0.251266) (-2.5,0.289301) (-2.4,0.31403) (-2.3,0.326564) (-2.2,0.328661) (-2.1,0.322366) (-2.,0.30973) (-1.9,0.292641) (-1.8,0.272713) (-1.7,0.251263) (-1.6,0.22931) (-1.5,0.207614) (-1.4,0.186715) (-1.3,0.166968) (-1.2,0.148589) (-1.1,0.131688) (-1.,0.116295) (-0.9,0.102389) (-0.8,0.0899073) (-0.7,0.0787655) (-0.6,0.0688653) (-0.5,0.060103) (-0.4,0.052373) (-0.3,0.0455729) (-0.2,0.0396055) (-0.1,0.0343794) (0.,0.0298108) (0.1,0.0258229) (0.2,0.0223469) (0.3,0.0193202) (0.4,0.0166876) (0.5,0.0143997) (0.6,0.0124129) (0.7,0.0106887) (0.8,0.00919323) (0.9,0.00789686) (1.,0.00677352) (1.1,0.00580053) (1.2,0.00495806) (1.3,0.00422879) (1.4,0.00359768) (1.5,0.00305166) (1.6,0.00257935) (1.7,0.00217085) (1.8,0.00181761) (1.9,0.0015122) (2.,0.00124817) (2.1,0.00101994) (2.2,0.000822668) (2.3,0.000652173) (2.4,0.000504831) (2.5,0.000377507) (2.6,0.000267488) (2.7,0.000172424) (2.8,0.0000902862) (2.9,0.0000193209) (3.,-0.0000419886) (3.1,-0.0000949567) (3.2,-0.000140716) (3.3,-0.000180246) (3.4,-0.000214394) (3.5,-0.000243894) (3.6,-0.000269378) (3.7,-0.000291391) (3.8,-0.000310406) (3.9,-0.000326831) (4.,-0.000341019) (4.1,-0.000353274) (4.2,-0.00036386) (4.3,-0.000373005) (4.4,-0.000380902) (4.5,-0.000387724) (4.6,-0.000393617) (4.7,-0.000398707) (4.8,-0.000403104) (4.9,-0.000406901) (5.,-0.00041018) (5.1,-0.000413015) (5.2,-0.000415461) (5.3,-0.000417575) (5.4,-0.000419401) (5.5,-0.000420977) (5.6,-0.00042234) (5.7,-0.000423516) (5.8,-0.000424533) (5.9,-0.00042541) (6.,-0.000426168) (6.1,-0.000426823) (6.2,-0.000427389) (6.3,-0.000427877) (6.4,-0.0004283) (6.5,-0.000428662) (6.6,-0.000428978) (6.7,-0.000429251) (6.8,-0.000429484) (6.9,-0.000429688) (7.,-0.000429862) (7.1,-0.000430014) (7.2,-0.000430145) (7.3,-0.000430258) (7.4,-0.000430356) (7.5,-0.000430439) (7.6,-0.000430512) (7.7,-0.000430576) (7.8,-0.000430629) (7.9,-0.000430678) (8.,-0.000430717) (8.1,-0.000430752) (8.2,-0.000430782) (8.3,-0.000430808) (8.4,-0.000430832) (8.5,-0.00043085) (8.6,-0.000430867) (8.7,-0.000430881) (8.8,-0.000430894) (8.9,-0.000430905) (9.,-0.000430914) (9.1,-0.000430923) (9.2,-0.000430929) (9.3,-0.000430936) (9.4,-0.00043094) (9.5,-0.000430945) (9.6,-0.000430949) (9.7,-0.000430952) (9.8,-0.000430955) (9.9,-0.000430957) (10.,-0.000430961) 
};

% Final RV 8.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.00384289) (-9.9,0.00382781) (-9.8,0.00380978) (-9.7,0.00378903) (-9.6,0.00376573) (-9.5,0.00373821) (-9.4,0.00370624) (-9.3,0.0036695) (-9.2,0.00362675) (-9.1,0.00357724) (-9.,0.00352025) (-8.9,0.00345403) (-8.8,0.0033775) (-8.7,0.00328901) (-8.6,0.00318609) (-8.5,0.00306698) (-8.4,0.00293006) (-8.3,0.00277016) (-8.2,0.00258645) (-8.1,0.00237366) (-8.,0.00212712) (-7.9,0.0018421) (-7.8,0.00151218) (-7.7,0.00113066) (-7.6,0.000689816) (-7.5,0.000180139) (-7.4,-0.000409576) (-7.3,-0.0010912) (-7.2,-0.00187797) (-7.1,-0.00278772) (-7.,-0.00383814) (-6.9,-0.00505051) (-6.8,-0.0064508) (-6.7,-0.00806507) (-6.6,-0.00992674) (-6.5,-0.0120707) (-6.4,-0.0145409) (-6.3,-0.017383) (-6.2,-0.0206491) (-6.1,-0.0244009) (-6.,-0.0287044) (-5.9,-0.0336341) (-5.8,-0.039272) (-5.7,-0.04571) (-5.6,-0.0530439) (-5.5,-0.0613782) (-5.4,-0.0708242) (-5.3,-0.0814933) (-5.2,-0.0934951) (-5.1,-0.106936) (-5.,-0.121902) (-4.9,-0.138457) (-4.8,-0.156623) (-4.7,-0.176362) (-4.6,-0.197548) (-4.5,-0.219947) (-4.4,-0.243166) (-4.3,-0.266627) (-4.2,-0.289514) (-4.1,-0.310735) (-4.,-0.328897) (-3.9,-0.342308) (-3.8,-0.34901) (-3.7,-0.346905) (-3.6,-0.333951) (-3.5,-0.308458) (-3.4,-0.269464) (-3.3,-0.217124) (-3.2,-0.152994) (-3.1,-0.0801028) (-3.,-0.00270159) (-2.9,0.074293) (-2.8,0.146042) (-2.7,0.208504) (-2.6,0.258935) (-2.5,0.296059) (-2.4,0.319957) (-2.3,0.331742) (-2.2,0.33317) (-2.1,0.326279) (-2.,0.313117) (-1.9,0.295565) (-1.8,0.275231) (-1.7,0.253424) (-1.6,0.23116) (-1.5,0.209193) (-1.4,0.188057) (-1.3,0.168104) (-1.2,0.149546) (-1.1,0.132489) (-1.,0.116961) (-0.9,0.102938) (-0.8,0.0903548) (-0.7,0.0791251) (-0.6,0.0691488) (-0.5,0.0603206) (-0.4,0.0525336) (-0.3,0.0456843) (-0.2,0.0396742) (-0.1,0.0344112) (0.,0.0298108) (0.1,0.0257954) (0.2,0.0222956) (0.3,0.0192484) (0.4,0.016598) (0.5,0.0142948) (0.6,0.0122947) (0.7,0.0105591) (0.8,0.00905374) (0.9,0.00774884) (1.,0.00661813) (1.1,0.00563878) (1.2,0.0047908) (1.3,0.0040568) (1.4,0.00342158) (1.5,0.00287201) (1.6,0.00239665) (1.7,0.00198551) (1.8,0.00162999) (1.9,0.00132261) (2.,0.00105688) (2.1,0.000827175) (2.2,0.000628638) (2.3,0.000457043) (2.4,0.000308759) (2.5,0.000180619) (2.6,0.0000698931) (2.7,-0.0000257826) (2.8,-0.000108447) (2.9,-0.000179867) (3.,-0.000241571) (3.1,-0.000294876) (3.2,-0.000340928) (3.3,-0.000380713) (3.4,-0.000415083) (3.5,-0.000444768) (3.6,-0.000470415) (3.7,-0.000492572) (3.8,-0.000511705) (3.9,-0.000528235) (4.,-0.000542514) (4.1,-0.00055485) (4.2,-0.000565504) (4.3,-0.000574704) (4.4,-0.000582655) (4.5,-0.000589519) (4.6,-0.00059545) (4.7,-0.000600573) (4.8,-0.000604997) (4.9,-0.000608819) (5.,-0.000612121) (5.1,-0.000614972) (5.2,-0.000617435) (5.3,-0.000619561) (5.4,-0.000621399) (5.5,-0.000622986) (5.6,-0.000624357) (5.7,-0.00062554) (5.8,-0.000626564) (5.9,-0.000627446) (6.,-0.00062821) (6.1,-0.000628868) (6.2,-0.000629438) (6.3,-0.000629929) (6.4,-0.000630353) (6.5,-0.000630721) (6.6,-0.000631038) (6.7,-0.00063131) (6.8,-0.000631549) (6.9,-0.000631751) (7.,-0.000631926) (7.1,-0.00063208) (7.2,-0.000632211) (7.3,-0.000632326) (7.4,-0.000632423) (7.5,-0.000632509) (7.6,-0.00063258) (7.7,-0.000632645) (7.8,-0.000632699) (7.9,-0.000632747) (8.,-0.000632786) (8.1,-0.000632824) (8.2,-0.000632853) (8.3,-0.000632878) (8.4,-0.000632903) (8.5,-0.000632922) (8.6,-0.000632938) (8.7,-0.000632953) (8.8,-0.000632965) (8.9,-0.000632978) (9.,-0.000632985) (9.1,-0.000632993) (9.2,-0.000633001) (9.3,-0.000633007) (9.4,-0.000633012) (9.5,-0.000633016) (9.6,-0.000633019) (9.7,-0.000633024) (9.8,-0.000633027) (9.9,-0.00063303) (10.,-0.000633032) 
};

% Final RV 9.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,0.0541278) (-9.9,0.0541121) (-9.8,0.0540941) (-9.7,0.0540731) (-9.6,0.0540494) (-9.5,0.0540211) (-9.4,0.0539891) (-9.3,0.0539516) (-9.2,0.0539083) (-9.1,0.0538581) (-9.,0.0538002) (-8.9,0.053733) (-8.8,0.0536553) (-8.7,0.0535656) (-8.6,0.0534612) (-8.5,0.0533403) (-8.4,0.0532012) (-8.3,0.0530394) (-8.2,0.0528527) (-8.1,0.0526367) (-8.,0.0523869) (-7.9,0.0520976) (-7.8,0.0517631) (-7.7,0.051376) (-7.6,0.0509285) (-7.5,0.0504113) (-7.4,0.049813) (-7.3,0.0491213) (-7.2,0.0483224) (-7.1,0.0473994) (-7.,0.0463331) (-6.9,0.0451026) (-6.8,0.0436816) (-6.7,0.0420434) (-6.6,0.0401537) (-6.5,0.0379769) (-6.4,0.0354693) (-6.3,0.0325844) (-6.2,0.0292678) (-6.1,0.0254582) (-6.,0.0210877) (-5.9,0.0160806) (-5.8,0.0103527) (-5.7,0.00381184) (-5.6,-0.00364151) (-5.5,-0.012114) (-5.4,-0.0217187) (-5.3,-0.0325707) (-5.2,-0.0447837) (-5.1,-0.0584669) (-5.,-0.0737121) (-4.9,-0.0905875) (-4.8,-0.10912) (-4.7,-0.129279) (-4.6,-0.150947) (-4.5,-0.173894) (-4.4,-0.197739) (-4.3,-0.22191) (-4.2,-0.245602) (-4.1,-0.267733) (-4.,-0.286921) (-3.9,-0.301483) (-3.8,-0.30947) (-3.7,-0.308794) (-3.6,-0.297415) (-3.5,-0.273644) (-3.4,-0.236514) (-3.3,-0.186166) (-3.2,-0.124133) (-3.1,-0.053411) (-3.,0.0217846) (-2.9,0.0965804) (-2.8,0.166178) (-2.7,0.226575) (-2.6,0.275053) (-2.5,0.310359) (-2.4,0.332584) (-2.3,0.342846) (-2.2,0.342897) (-2.1,0.334772) (-2.,0.320508) (-1.9,0.301977) (-1.8,0.280775) (-1.7,0.258203) (-1.6,0.235265) (-1.5,0.212707) (-1.4,0.191053) (-1.3,0.170646) (-1.2,0.151692) (-1.1,0.13429) (-1.,0.118461) (-0.9,0.104176) (-0.8,0.0913655) (-0.7,0.0799383) (-0.6,0.0697906) (-0.5,0.0608137) (-0.4,0.0528978) (-0.3,0.0459369) (-0.2,0.0398302) (-0.1,0.0344836) (0.,0.0298108) (0.1,0.0257328) (0.2,0.0221788) (0.3,0.0190848) (0.4,0.016394) (0.5,0.0140558) (0.6,0.0120255) (0.7,0.0102638) (0.8,0.00873588) (0.9,0.00741147) (1.,0.00626391) (1.1,0.00527002) (1.2,0.00440946) (1.3,0.0036646) (1.4,0.00302) (1.5,0.00246233) (1.6,0.00197997) (1.7,0.00156278) (1.8,0.00120204) (1.9,0.000890149) (2.,0.00062052) (2.1,0.000387453) (2.2,0.000186005) (2.3,0.0000119062) (2.4,-0.000138549) (2.5,-0.000268564) (2.6,-0.000380907) (2.7,-0.000477979) (2.8,-0.00056185) (2.9,-0.000634312) (3.,-0.000696915) (3.1,-0.000751) (3.2,-0.000797724) (3.3,-0.000838086) (3.4,-0.000872955) (3.5,-0.000903076) (3.6,-0.000929097) (3.7,-0.000951574) (3.8,-0.000970989) (3.9,-0.00098776) (4.,-0.00100225) (4.1,-0.00101476) (4.2,-0.00102557) (4.3,-0.00103491) (4.4,-0.00104297) (4.5,-0.00104994) (4.6,-0.00105595) (4.7,-0.00106115) (4.8,-0.00106564) (4.9,-0.00106952) (5.,-0.00107287) (5.1,-0.00107576) (5.2,-0.00107826) (5.3,-0.00108041) (5.4,-0.00108228) (5.5,-0.00108389) (5.6,-0.00108528) (5.7,-0.00108648) (5.8,-0.00108752) (5.9,-0.00108841) (6.,-0.00108919) (6.1,-0.00108986) (6.2,-0.00109043) (6.3,-0.00109093) (6.4,-0.00109136) (6.5,-0.00109174) (6.6,-0.00109206) (6.7,-0.00109234) (6.8,-0.00109258) (6.9,-0.00109278) (7.,-0.00109296) (7.1,-0.00109312) (7.2,-0.00109325) (7.3,-0.00109337) (7.4,-0.00109346) (7.5,-0.00109355) (7.6,-0.00109362) (7.7,-0.00109369) (7.8,-0.00109374) (7.9,-0.00109379) (8.,-0.00109383) (8.1,-0.00109387) (8.2,-0.0010939) (8.3,-0.00109393) (8.4,-0.00109395) (8.5,-0.00109397) (8.6,-0.00109399) (8.7,-0.001094) (8.8,-0.00109401) (8.9,-0.00109403) (9.,-0.00109403) (9.1,-0.00109404) (9.2,-0.00109405) (9.3,-0.00109406) (9.4,-0.00109406) (9.5,-0.00109407) (9.6,-0.00109407) (9.7,-0.00109407) (9.8,-0.00109408) (9.9,-0.00109408) (10.,-0.00109408) 
};

% Final RV 10.
\addplot[color=red, thin, mark=none] plot coordinates {
(-10.,-0.0166538) (-9.9,-0.0166692) (-9.8,-0.0166872) (-9.7,-0.016708) (-9.6,-0.0167314) (-9.5,-0.0167594) (-9.4,-0.0167912) (-9.3,-0.0168285) (-9.2,-0.0168713) (-9.1,-0.0169211) (-9.,-0.0169787) (-8.9,-0.0170453) (-8.8,-0.0171222) (-8.7,-0.0172111) (-8.6,-0.0173147) (-8.5,-0.0174346) (-8.4,-0.0175725) (-8.3,-0.017733) (-8.2,-0.0179181) (-8.1,-0.0181322) (-8.,-0.0183799) (-7.9,-0.0186667) (-7.8,-0.0189985) (-7.7,-0.0193823) (-7.6,-0.0198259) (-7.5,-0.0203386) (-7.4,-0.0209318) (-7.3,-0.0216175) (-7.2,-0.0224095) (-7.1,-0.0233246) (-7.,-0.0243814) (-6.9,-0.025601) (-6.8,-0.0270094) (-6.7,-0.0286331) (-6.6,-0.0305057) (-6.5,-0.0326627) (-6.4,-0.0351473) (-6.3,-0.0380052) (-6.2,-0.0412906) (-6.1,-0.0450637) (-6.,-0.0493915) (-5.9,-0.0543489) (-5.8,-0.0600187) (-5.7,-0.0664914) (-5.6,-0.0738649) (-5.5,-0.0822439) (-5.4,-0.0917388) (-5.3,-0.102462) (-5.2,-0.114522) (-5.1,-0.128026) (-5.,-0.143059) (-4.9,-0.159683) (-4.8,-0.177918) (-4.7,-0.197723) (-4.6,-0.218969) (-4.5,-0.241415) (-4.4,-0.264661) (-4.3,-0.288116) (-4.2,-0.310953) (-4.1,-0.332061) (-4.,-0.350029) (-3.9,-0.363138) (-3.8,-0.369403) (-3.7,-0.3667) (-3.6,-0.352959) (-3.5,-0.32647) (-3.4,-0.286262) (-3.3,-0.232498) (-3.2,-0.166762) (-3.1,-0.0921295) (-3.,-0.0129195) (-2.9,0.0658764) (-2.8,0.139345) (-2.7,0.203382) (-2.6,0.255198) (-2.5,0.293495) (-2.4,0.31835) (-2.3,0.330887) (-2.2,0.332884) (-2.1,0.326407) (-2.,0.313531) (-1.9,0.296162) (-1.8,0.275933) (-1.7,0.254173) (-1.6,0.231914) (-1.5,0.209922) (-1.4,0.188743) (-1.3,0.168733) (-1.2,0.150113) (-1.1,0.132991) (-1.,0.117399) (-0.9,0.103314) (-0.8,0.0906714) (-0.7,0.0793871) (-0.6,0.0693606) (-0.5,0.0604867) (-0.4,0.0526585) (-0.3,0.0457722) (-0.2,0.0397292) (-0.1,0.0344371) (0.,0.0298108) (0.1,0.0257726) (0.2,0.0222527) (0.3,0.019188) (0.4,0.0165222) (0.5,0.0142056) (0.6,0.0121938) (0.7,0.0104479) (0.8,0.00893367) (0.9,0.00762102) (1.,0.00648359) (1.1,0.0054984) (1.2,0.00464535) (1.3,0.00390694) (1.4,0.00326792) (1.5,0.00271505) (1.6,0.00223681) (1.7,0.0018232) (1.8,0.00146553) (1.9,0.0011563) (2.,0.000888957) (2.1,0.000657865) (2.2,0.000458122) (2.3,0.000285493) (2.4,0.000136307) (2.5,0.00000738862) (2.6,-0.00010401) (2.7,-0.000200265) (2.8,-0.00028343) (2.9,-0.000355285) (3.,-0.000417362) (3.1,-0.000470993) (3.2,-0.000517325) (3.3,-0.00055735) (3.4,-0.000591926) (3.5,-0.000621795) (3.6,-0.0006476) (3.7,-0.000669887) (3.8,-0.000689141) (3.9,-0.000705772) (4.,-0.000720135) (4.1,-0.000732545) (4.2,-0.000743264) (4.3,-0.000752523) (4.4,-0.000760518) (4.5,-0.000767426) (4.6,-0.000773395) (4.7,-0.000778549) (4.8,-0.000783) (4.9,-0.000786843) (5.,-0.000790163) (5.1,-0.000793035) (5.2,-0.000795511) (5.3,-0.000797651) (5.4,-0.000799502) (5.5,-0.000801095) (5.6,-0.000802475) (5.7,-0.000803668) (5.8,-0.000804697) (5.9,-0.000805584) (6.,-0.000806352) (6.1,-0.000807015) (6.2,-0.000807588) (6.3,-0.000808083) (6.4,-0.00080851) (6.5,-0.000808878) (6.6,-0.000809199) (6.7,-0.000809473) (6.8,-0.00080971) (6.9,-0.000809917) (7.,-0.000810091) (7.1,-0.000810244) (7.2,-0.000810377) (7.3,-0.000810492) (7.4,-0.000810593) (7.5,-0.000810675) (7.6,-0.000810751) (7.7,-0.000810815) (7.8,-0.000810868) (7.9,-0.000810918) (8.,-0.000810959) (8.1,-0.000810995) (8.2,-0.000811024) (8.3,-0.00081105) (8.4,-0.000811074) (8.5,-0.000811092) (8.6,-0.00081111) (8.7,-0.000811125) (8.8,-0.000811139) (8.9,-0.00081115) (9.,-0.000811156) (9.1,-0.000811166) (9.2,-0.000811171) (9.3,-0.00081118) (9.4,-0.000811182) (9.5,-0.00081119) (9.6,-0.000811193) (9.7,-0.000811194) (9.8,-0.000811197) (9.9,-0.000811203) (10.,-0.000811205) 
};


